\'Eliv\'agar: Efficient Quantum Circuit Search for Classification

Designing performant and noise-robust circuits for Quantum Machine Learning (QML) is challenging -- the design space scales exponentially with circuit size, and there are few well-supported guiding principles for QML circuit design. Although recent Quantum Circuit Search (QCS) methods attempt to search for performant QML circuits that are also robust to hardware noise, they directly adopt designs from classical Neural Architecture Search (NAS) that are misaligned with the unique constraints of quantum hardware, resulting in high search overheads and severe performance bottlenecks. We present \'Eliv\'agar, a novel resource-efficient, noise-guided QCS framework. \'Eliv\'agar innovates in all three major aspects of QCS -- search space, search algorithm and candidate evaluation strategy -- to address the design flaws in current classically-inspired QCS methods. \'Eliv\'agar achieves hardware-efficiency and avoids an expensive circuit-mapping co-search via noise- and device topology-aware candidate generation. By introducing two cheap-to-compute predictors, Clifford noise resilience and Representational capacity, \'Eliv\'agar decouples the evaluation of noise robustness and performance, enabling early rejection of low-fidelity circuits and reducing circuit evaluation costs. Due to its resource-efficiency, \'Eliv\'agar can further search for data embeddings, significantly improving performance. Based on a comprehensive evaluation of \'Eliv\'agar on 12 real quantum devices and 9 QML applications, \'Eliv\'agar achieves 5.3% higher accuracy and a 271$\times$ speedup compared to state-of-the-art QCS methods.

==> asplos24-extended-abstract-template.tex <==

%replace XXX with the submission number you are given from the ASPLOS submission site.
\newcommand{\asplossubmissionnumber}{XXX}

\usepackage[normalem]{ulem}

\begin{document}

\title{Your Paper Title \\ \textbf{Extended Abstract}}

\date{}

\maketitle

\thispagestyle{empty}

% No abstract needed for the extended abstract
%\begin{abstract}
%\end{abstract}


ASPLOS'24 will require the submission of {\it Extended
Abstracts}. Your extended abstract --- inspired by the model used for
IEEE Micro Top
Picks --- should be {\it two pages long}, and it will be submitted separately
from your main paper. The deadline for the extended abstract and the
full paper will be identical. Except for the page limit, \textbf{all other
formatting and anonymity requirements are identical} to those for full
papers: no names or affiliations should be present, and citations should
be anonymized if appropriate. Extended abstracts should be self-contained, though they may
contain references to the full paper.

We \emph{recommend}---but do not require--- that you use
the following organization for your abstract. 
Sections~\ref{sec:motivation} through \ref{sec:key-contributions}
should be a summary of your full paper. Section~\ref{sec:motivation}
motivates the paper; Section~\ref{sec:limitations} describes
limitations of the state of the art, if applicable;
Section~\ref{sec:key-insights} presents the key new insight or
insights of the paper; 
Section~\ref{sec:main-artifacts} presents the main artifacts described
in the paper;  Section~\ref{sec:key-contributions} summarizes the key
results and technical contributions of your paper. Finally,
Section~\ref{sec:why-asplos} should explain why the paper is suitable
for ASPLOS. In
Section~\ref{sec:revisions}, you may optionally include a paragraph
describing how your paper has been revised, if it was previously
submitted to another conference.

The extended abstracts must be submitted in printable PDF format and should contain a
{\bf maximum of 2 pages} of single-spaced two-column text, {\bf not
  counting references}.  You may include any number of pages for
references, but we suggest you limit your bibliography to
only the most relevant references. The extended
abstracts should use the same formating as the regular papers. If you are using
\LaTeX~\cite{lamport94} to typeset your extended abstract, then we suggest that
you use the template that we provided on ASPLOS website.
If you use a different
software package, then please adhere to the formatting guidelines provided in the ASPLOS website.
For examples, please check the 
\href{https://asplos-conference.org/2021/index.html\%3Fp=2181.html}
{extended abstracts of papers accepted
by ASPLOS 2021}.

The references section of your extended abstract will not count
towards the two page limit. We suggest you limit your bibliography to
only the most relevant references~\cite{lamport94}.

The extended abstract should not have an abstract. Start with Section~\ref{sec:motivation}.

\section{Motivation}
\label{sec:motivation}


\begin{itemize}
\item What is the problem your work attacks? Be specific.
\item Why is it an important problem?
\end{itemize}

\vspace{1em}

\noindent
Articulate the importance of this problem to the broader ASPLOS
community, using as little jargon as possible. \emph{Be specific}
about the problem you are addressing; it should be the one that your
paper directly addresses.

\section{Limitations of the State of the Art}
\label{sec:limitations}

\begin{itemize}
\item What is the state of the art in this topic today (if any)?
\item What are its limits?
\end{itemize}

\section{Key Insights}
\label{sec:key-insights}

\begin{itemize}
\item What are the one or two key new insights in this paper?
\item How does it advance the state of the art?
\item What makes it more effective than past approaches?
\end{itemize}

\section{Main Artifacts}
\label{sec:main-artifacts}

\begin{itemize}
\item What are the key artifacts presented in your paper: a
  methodology, a hardware design, a software algorithm, an
  optimization or control technique, etc.?
  \item How were your artifacts implemented and evaluated? 
\end{itemize}

\section{Key Results and Contributions}
\label{sec:key-contributions}

\begin{itemize}
  \item What are the most important \emph{one or two} empirical or theoretical
    results of this approach?
  \item What are the contributions that this paper makes to the state of the
    art? List them in an \texttt{itemize} section. Each contribution should be no more than a few sentences long.
  \item Clearly describe its advantages over past work, including how it overcomes their limitations.
\end{itemize}


\section{Why ASPLOS}
\label{sec:why-asplos}

ASPLOS emphasizes multidisciplinary research; explain how this
  paper emphasizes synergy of \emph{two or more ASPLOS areas}: architecture,
  programming languages, operating systems, and related areas (broadly
  interpreted).

\noindent
If you are unsure whether your paper falls within the scope of ASPLOS,
please check with the program chairs -- ASPLOS is a broad,
multidisciplinary conference and encourages new topics.

%  \url{https://rb.gy/hd1hms}).

\section{Revisions}
\label{sec:revisions}

 \emph{Optional:} Describe how this paper has been revised, if it was previously submitted to another conference.

 
\pagebreak
\bibliographystyle{plain}
\bibliography{references}


\end{document}

==> v1/background.tex <==
%\newpage %%% do not move this--- I need to estimate the space
\section{Background}
\label{sec:background}
\subsection{Execution of Quantum Programs on NISQ Computers}
% To run a quantum program, compilers (1)~\textit{map} the program qubits on to the physical qubits of the target quantum device and (2)~\textit{translates} the high-level program instructions on to low-level device-compliant native gates. Unfortunately, noisy quantum devices and imperfections in quantum operations make program executions susceptible to computational errors. 

In the NISQ era, noisy quantum devices and imperfect quantum operations make  program executions susceptible to computational errors. Moreover, most NISQ devices are characterized by limited connectivity between qubits. To overcome this constraint, a circuit  \textit{routing} step is required for executing circuits of arbitrary topology, where quantum SWAP operations are used to relocate non-adjacent qubits so that 2-qubit gates can be performed between them, as shown in~\cref{fig:swap}. SWAP operations are usually implemented using 3 imperfect physical 2-qubit gates, and thus are expensive and error-prone. Prior works~\cite{murali2020crosstalk, das2021adapt, ravi2022cliffordcanarycircuits, tannu2022hammer} show that circuit fidelity can be improved by leveraging circuits that require less SWAP operations or with structures that are more robust to various device error sources.

% %\textbf{Circuit structure and mapping are key to noise robustness.} Previous works in quantum compilation~\cite{murali2020crosstalk, das2021adapt, ravi2022cliffordcanarycircuits, tannu2022hammer} have suggested that compiling the same circuit to different circuit structures with different scheduling, routing  and mapping methods can drastically alter the level of noise robustness. This shows that the structure and mapping of a circuit is highly impactful to noise robustness. However, due to the complexity of device noise sources and the competing constraints induced by different noise sources, there is no universal method to determine the  circuit structures and mapping strategies for optimal noise robustness on different quantum devices.

% \ignore{\textbf{NISQ devices are erroneous.} NISQ quantum devices suffer from high error rates when execute a quantum program. For example, qubit states are fragile and tend to interact with their environment~\cite{sycamoredatasheet}, which cause decoherence error and leak important quantum information.  In addition, imperfect quantum gates, measurement operations and cross-talk between gate control signals also reduce the reliability of the circuit output.

% \textbf{NISQ devices have limited connectivity.} In NISQ hardware, limited connectivity between qubits imposes constraints on the 2-qubit operations that can be performed on a device. As shown in~\cref{fig:swap}, if a circuit includes a 2-qubit gate applied onto a pair of qubits not directly connected on the device, SWAP gates must be inserted in order to enable the application of the gate. Since SWAP gates are constructed using 3 consecutive CNOT gates and CNOT gate error rates on current NISQ devices are about 1\%~\cite{sycamoredatasheet, IBMQ, acharya2022suppressing}, quantum SWAP gates not only increase circuit latency and further cause decoherence but also introduce more gate errors.}

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.99\textwidth]{figs/framework/overview@3x.png}
        
    \caption{An overview of \framework{}.}
    % \vspace*{-0.2cm}
    \label{fig:framework_overview}
\end{figure*}



%These constraints are because when a two-qubit operation applies to two qubits, those two qubits are required to be connected to each other on the device. Otherwise, compilers need to route the nonadjacent qubits adjacent to each other. To route qubits, CNOT gates are exploited which increase the depth of the circuits and are the dominant source of errors in executing circuits on NISQ devices~\cite{sycamoredatasheet}. Therefore, routing qubits increase the error on quantum circuits and significantly affect the fidelity of the output.


% \textbf{Circuit structure is determinant to noise robustness.} \YS{This has to be rewritten.} Previous works on quantum compilation have suggested that noise robustness can be improved by altering circuit structure and leveraging noise footprint on quantum devices, e.g., mapping circuits to qubits of better fidelity and scheduling quantum gates based on cross-talk errors.  However, due to the complexity of device noise sources and competing constraints between them, these policies are still far from optimal, it still remains unclear how circuit structures exactly relate to noise robustness.



%  (e.g., serialized circuits are  robust to cross-talk errors and parallelized circuits are robust to decoherence errors)

%\textbf{Circuit structure is a key determinant of noise robustness.} Previous works in quantum compilation such as~\cite{murali2020crosstalk, das2021adapt, ravi2022cliffordcanarycircuits, tannu2022hammer} have suggested that noise robustness can be improved by altering circuit structure, and that circuits with similar structure are noise robust to similar degrees. However, due to the complexity of device noise sources and the competing constraints induced by different noise sources, optimizing circuit fidelity is non-trival. Additionally, the exact causal relationships between circuit characteristics and output fidelity are still unclear, rendering current approaches far from optimal.


% Despite the effect of noise on the output of quantum circuits, we can design quantum circuits resilient to noise up to a level that faulty operations do not cause a computational failure~\cite{Preskill2018quantumcomputingin}. This emphasizes the importance of finding strategies to design quantum circuits that are inherently noise resilient, which is an effective alternative to unaffordably expensive error correction methods for near-term quantum devices.
 
\subsection{Quantum Machine Learning}
\label{sec:qml_intro}
%, shown in \cref{fig:qml}
% (1)~\textit{data embedding} in which the input training data is encoded into the quantum states manipulated by a variational circuit, 
\subsubsection{Variational circuits}
QML uses variational circuits to perform machine learning tasks. Variational circuits for QML consist of three parts: a trainable variational subcircuit, a set of data embedding gates, and a set of measurement operations. Trainable variational subcircuits often include parametric 1- and 2-qubit gates with trainable parameters (ex. \new{RY$(\theta)$}, where $\theta$ is a trainable parameter) and \new{optionally some non-parametric gates (ex. CX)}. Data embedding gates are used to encode classical data into quantum states that can be manipulated by variational circuits, and can be placed in arbitrary positions in a circuit. Measurement operations are performed on a subset of the qubits operated on by a circuit to obtain circuit outputs for further processing. 


\subsubsection{Data embedding gates}
\label{sec:data_embedding}

\imp{While current QCS methods focus on optimizing the variational portion of a QML circuit, the data embedding used is a key determinant of the performance of  variational circuits\cite{schuld2022fourierinterpolation, schuld2021encodingexpressivity, schuld2021qmlmodelsarekernelmethods, sweke2021encodingdependentbounds}. We use a simple 1-qubit example to illustrate their importance. \new{As seen in ~\cref{fig:embedding}, two 1-qubit variational circuits with the same parametric gates \new{(U3$(\vec{\theta_1})$ and U3$(\vec{\theta_2})$) but different embeddings (RX$(x)$ and RY$(x)$, versus RX$(x)$ only)} exhibit completely different performance when used to learn a simple sinusoidal function. The theory developed in~\cite{schuld2021encodingexpressivity, schuld2022fourierinterpolation} emphasizes the need to use a well-suited data embedding to accurately learn any target function. Thus, identifying such data embeddings for a given QML task is crucial for high performance.}}

Unfortunately, finding effective data embeddings is challenging due to the large search space. Existing QCS frameworks rely on fixed embedding schemes, such as an angle embedding~\cite{qml} or an IQP embedding~\cite{havlek2019suplearninginquantumenhancedfeaturespaces}, and place these embedding gates in the beginning of every candidate circuit for all QML tasks, leading to potentially poor performance due to the mismatch between the \new{QML task} and the embedding.
\subsubsection{Training variational circuits}

To perform machine learning tasks, variational circuits need to be trained. As illustrated in~\cref{fig:qml}, the training process of variational circuits involves iterating between circuit executions and a classical optimization algorithm. 
% Typically, variational circuits are executed to evaluate the gradients of circuit parameters, which are then used by a classical gradient-based optimizer to update circuit parameter values.

% Training a variational circuit is more expensive than training a classical ML model due to the increased cost of gradient computation on quantum hardware. Classically, gradients can be computed in constant time via Automatic Differentiation (AD)~\cite{ad_survey}. However, AD is not feasible on quantum computers because the backpropagation step in AD requires intermediate states being used but measuring intermediate quantum states will destroy them~\cite{NielsenChuang}. Moreover, these intermediate states cannot be copied due to the no-cloning property~\cite{nocloning}. Thus, gradient-based optimization for QML requires algebraic methods such as parameter-shift rules \cite{schuld2019analyticgradients, wierichs2022parametershift} for computing gradients. Parameter-shift rule based methods evaluate the gradient of a single parameter $\theta$ by running two circuits with shifted parameters $\theta+s$ and $\theta-s$, respectively ($s$ is a constant), and computing the difference the two circuit outputs. The number of circuit executions is linear in the number of circuit parameters, as opposed to the constant scaling of AD methods. Thus, computing gradients in QML scales poorly with circuit size. Current QCS methods use SuperCircuit-based candidate evaluation strategies which rely heavily on gradient computation, and so inherit this unfavourable scaling, leading to a large training costs.

Training a variational circuit is more expensive than training a classical ML model due to the increased cost of gradient computation on quantum hardware. Classically, gradients can be computed in constant time via Automatic Differentiation (AD)~\cite{ad_survey}. \new{However, AD is not feasible on quantum computers since intermediate quantum states cannot be manipulated or copied~\cite{NielsenChuang, nocloning}}. Thus, gradient-based optimization for QML requires algebraic methods such as parameter-shift rules \cite{schuld2019analyticgradients, wierichs2022parametershift} for computing gradients. Parameter-shift rule based methods evaluate the gradient of a single parameter $\theta$ by running two circuits with shifted parameters $\theta+s$ and $\theta-s$, respectively ($s$ is a constant), and computing the difference the two circuit outputs. The number of circuit executions is linear in the number of circuit parameters, as opposed to the constant scaling of AD methods. Thus, computing gradients in QML scales poorly with circuit size. Current QCS methods use SuperCircuit-based candidate evaluation strategies which rely heavily on gradient computation, and so inherit this unfavourable scaling, leading to large training costs.

% \ignore{
% The most expensive 

%  QML has two phases: (1)~\textit{training} during which parameters of variational circuits are updated using classical optimization algorithms, such as gradient descent, and (2)~\textit{inference} during which the trained circuit is used to perform an ML task on an unseen data. 


% Although promising, designing (1)~\textit{efficient} QML circuits that fits the training data and accurately classifies unseen data (2)~while being robust to quantum device errors remain a challenge due to the lack of well-defined templates for designing such circuits. While manually crafted circuits optimize across both these dimensions for small problems, scaling such methods to practical problem sizes is non-trivial.  
% % QML algorithms consist of two components: a variational circuit and a classical optimizer. There are also two phases in QML algorithms: training and inference. In the training phase, the variational circuit and the classical optimizer work together in iterations: the circuit provides the gradients of circuit parameters to the classical optimizer, and the classical optimizer guides the updates 

% \subsubsection{Reliance on device-agnostic searches}
% \subsubsection{Overlook the impact of data embedding}
% \label{sec:data_embedding}
% Data embedding is the process of encoding classical data into quantum states by using a set of data-dependent parameterized quantum gates and is a vital step that impacts the performance of QML circuits. 
% \ignore{
% To perform quantum operations on classical data, we require to encode them to quantum data, which referred to as data embedding or quantum feature map. Unlike feature maps in classical ML, encoding classical data to quantum data and transfer all the requiring to the quantum setting is not trivial. At the same time, Embedding is a critical part of a QML model as prior works~\cite{lloyd2020quantum,schuld2021encodingexpressivity} show that effective embedding significantly increase the performance of QML models for a given machine learning task. }For example, Fig.~\ref{fig:embedding} shows that for the same  VQC, different embeddings result in different accuracies in fitting the data. 

% \subsubsection{Expensive training costs}
% \label{sec:gradient}
% To update each parameter $\theta$ during training, QML uses the parameter-shift rule that calculates the derivative of parameter $\theta$ by running two circuits, one with $\theta+s$ and the other one with $\theta-s$, and computing the difference between the expectation values of their outputs. Thus, we requires $2NM$ circuit evaluations, for a QML model with $N$ parameters and a dataset of size $M$. As prior QCS frameworks perform all these evaluations on real NISQ devices, they are extremely \textit{resource inefficient}. 

% }
% \subsubsection{VQCs as partial Fourier series}

% \begin{figure}[t]
%     \centering
        
%     \begin{subfigure}{0.8\columnwidth}
%         \centering
%         \includegraphics[width=1\columnwidth]{figs/introduction/circs@3x.png}
%         \caption{}
%         \label{fig:embedding_circs}
%     \end{subfigure}
      
%     \begin{subfigure}{1\columnwidth}
%         \centering
%         \includegraphics[width=0.8\columnwidth]{figs/introduction/3c@3x.png}
%         \caption{}
%         \label{fig:embedding_funcs}   
         
%     \end{subfigure}
 
%     \caption{\YS{make it 2 columns, (1) swap (2) qml (3) embedding}\textbf{Effect of data embedding on the performance of QML models in fitting a dataset} (a) Two QML circuits that both have the same trainable subcircuits but different data embeddings. Circuit 1 uses an \( RX \) and an \( RY \) gate to embed the input data, and Circuit 2 uses only an \( RX \) embedding gate. (b) Predictions made by Circuits 1 and 2 after training on points sampled from \( f(x) = -0.75\sin{2x} + 0.05\). Circuit 2 fails to learn $f$ due to its unoptimized data embedding.}
%     \label{fig:embeddings}
%     % \vspace*{-0.7cm}
% \end{figure}


% \cite{schuld2021encodingexpressivity, schuld2022fourierinterpolation} showed that the outputs of VQCs can be represented using partial Fourier series in the input data. The set of Fourier frequencies and the values of the coefficients determining the relative weight of each frequency in the output of a VQC is largely determined by the choice of data embedding used.Thus, tailoring the embedding used in a VQC based on the input data can lead to dramatically improved performance on QML tasks. \cref{fig:embeddings} illustrates this using a simple 1-qubit example.



% \ignore{

% \subsection{Limitations of Prior Quantum Circuit Search Frameworks}
% \ignore{\color{red}{talk little about tool-chains that automatically attempt to achieve the goals in one line. then tell they have the following limitations}}
% Prior Quantum Circuit Search (QCS) frameworks that search for QML circuits~\cite{wang2021quantumnas,dacheng2020quantumsupernet,hong2020dqas} do not consider the constraints of NISQ devices or poorly address their constraints as they do not decouple the effects of hardware-level and software-level challenges in their design. The drawbacks of prior QCS frameworks are:


% To calculate the partial derivatives of circuit parameters during the training of QML, the classical methods, such as automatic differentiation~\cite{baydin2015autodiffsurvey}, are infeasible on quantum hardware. This is because we cannot calculate the derivative of intermediate states of quantum systems without measurement which changes the quantum state. Work~\cite{schuld2019analyticgradients} addresses this challenge by introducing the parameter-shift rule that calculates the derivative w.r.t parameter $\theta$ by running two circuits, one with $\theta+s$ and the other one with $\theta-s$. The partial derivative of $\theta$ is the difference between the expectation value of measurement results of these two circuits. Based on this method, training a QML model with $N$ number of trainable parameters using a dataset of size $M$, requires running $2NM$ different circuits on the device, which is a costly process especially as dataset size $M$ is a comparably large number.

% }

% \ignore{
% \subsection{Current QCS methods and limitation}
% \label{sec:nas_intro}

% \YS{Differences between NQCS and cNAS: (1) Evaluation is more expensive on NQCS and the performance bottleneck (2) Need to respect noise and topology (3) data embedding}
% Since the seminal work of \cite{quoc2016rlnas}, various cNAS methods have been proposed. All of these methods can be categorized using the decomposition presented in \cite{elsken2018nassurvey}:

% \begin{itemize}
%     \item \textbf{Search space:} what kind of operations, structure and connections can valid candidate architectures use?
%     \item \textbf{Search algorithm:} how do we generate new candidate architectures from the chosen search space?
%     \item \textbf{Candidate evaluation strategy:} how do we measure the performance of candidate architectures on the target task?
% \end{itemize}

% Popular cNAS search spaces are defined using cell-based representations \cite{yi2020nb201, radosavovic202nds}, or the architecture of the supernet used \cite{dean2018classicalsupernet, pham2018enas}. Prevalent search algorithms include random search \cite{he2019randomlywired, mellor2020naswot}, evolutionary search \cite{quoc2018evosearchnas}, gradient descent \cite{liu2018darts, shu2021nasi}, reinforcement learning \cite{quoc2016rlnas, baker2016rlnas}, and pruning-based methods \cite{chen2021tenas}. Current candidate evaluation strategies can be largely classified into one of two categories: one-shot methods \cite{dean2018classicalsupernet, pham2018enas}, which require the training of a large supernet, or zero-shot methods \cite{shu2021nasi, mellor2020naswot, chen2021tenas, abdelfattah2021zerocostproxies}, which aim to estimate the performance of a candidate architecture on an ML task without performing any training, often using a single mini-batch of data to estimate performance.

% % Many cNAS search spaces \cite{hutter2019nb101}, \cite{yi2020nb201}) use a cell-based representation of the search space. Candidate architectures are constructed by inserting multiple copies of a cell into slots in a predefined neural network backbone; variations in architectures are solely due to difference between the cells used to construct the networks. Other works such as \cite{dean2018classicalsupernet} choose to use a supernet, a large directed acylic graph which contains all possible candidate architectures as subgraphs. Some early works (\cite{quoc2016rlnas}, \cite{baker2016rlnas}) use a search space where candidate architectures are constructed by stacking multiple layer-wise operations in a sequential manner, but this approach is rarely used today, since it covers far larger search spaces, making it intractable to cover the entire search space, and a significant amount of expert knowledge in order to design performant search spaces. 

% % \emptyline

% % Prevalent search strategies include using a reinforcement learning controller that learns to propose good candidate architectures (\cite{quoc2016rlnas}, \cite{baker2016rlnas}), evolutionary search \cite{quoc2018evosearchnas}, gradient descent over a parametrized distribution covering the search space (darts, find one more), and random search ((simplfiying one shot NAS paper, \cite{mellor2020naswot}).

% % \emptyline

% % The most costly phase of NAS is candidate evaluation: early works (\cite{quoc2016rlnas}, \cite{baker2016rlnas}) trained sampled candidate architectures to convergence on the target learning task, providing an accurate but extremely costly estimate of candidate performance, with the experiments reported in the paper taking over 200,000 GPU hours to complete. \cite{dean2018classicalsupernet} introduced the idea of parameter sharing, where candidate architectures that use similar operations also use the same learned weights for these operations. This drastically reduces the training time required, often by multiple orders of magnitude, but results in a less accurate estimation of candidate performance. There is evidence that weight sharing approaches might not outperform random search on common NAS image classification and language modelling tasks \cite{yu2020classicalnassurvey, li2019nassurvey} due to the unreliability of the performance of architectures using shared parameters as a performance estimator. More recently, works such as \cite{mellor2020naswot}, (zero shot survey), (TE Nas), (NASI), have tried to further reduce the search time required by avoiding training altogether by using a zero-shot proxy for the performance of candidate architectures. These proxies are usually computed by examining the gradients, activations, or outputs of a randomly initialized network for a minibatch of data. An orthogonal line of work aims to use a trained neural network as a predictor for the performance of candidate architectures (add some references), which do not require candidate networks to be trained, but need a large dataset of trained networks in order to learn from in order to accurately estimate candidate performance.


% \subsection{Current approaches to NQCS}

% NQCS is largely similar to cNAS, with one key difference: NQCS methods must use candidate evaluation strategies that not only measure candidate performance on the QML task of interest, but also their robustness to hardware noise on the device the returned circuit is to be deployed on. Early NQCS works such as \cite{chen2021rlqas, dunjko2021rlqas, yao2021neuralpredictorqas}, only focused on QAOA and VQE problems. More recently, QuantumSupernet \cite{dacheng2020quantumsupernet} and QuantumNAS \cite{wang2021quantumnas} applied NQCS methods to classification problems using classical data, such as MNIST \cite{} and FMNIST \cite{}.

% Current NQCS methods are largely based on prevalent techniques in cNAS. For example, QuantumSupernet and QuantumNAS use search algorithms and candidate evaluation strategies derived from classical supernet formulations ~\cite{pham2018enas, dean2018classicalsupernet}. QuantumNAS additionally uses an evolutionary algorithm akin to those proposed in ~\cite{quoc2018evosearchnas} to co-search for a VQC and qubit mapping. The search algorithm and candidate evaluation strategy in DQAS are inspired by the classical DARTS framework ~\cite{liu2018darts}, which enables navigation of the search space via gradient descent. 


% \subsection{Limitations of current NQCS approaches}
% \label{sec:limitation_current}

% \begin{enumerate}
    
%     \item \textbf{Classically-inspired candidate evaluation strategies are expensive to compute on quantum computers:} Candidate evaluation in cNAS relies heavily on gradient computation \cite{ning2020classicalnassurvey, abdelfattah2021zerocostproxies, chen2021tenas, shu2021nasi, pham2018enas, dean2018classicalsupernet}, which can be computed in constant time classically via automatic differentiation.  However, gradient computation on quantum hardware requires the parameter shift rule  \cite{schuld2019analyticgradients, wierichs2022parametershift} or finite difference methods \TD{improve, give intuition}, which takes time linear in the parameter count of a VQC. Thus, the classically-inspired evaluation strategies in current NQCS methods incur large evaluation costs and scale poorly with circuit size. Furthermore, current NQCS methods conflate circuit intrinsic performance and noise robustness by directly measuring performance on the target device. Evaluating noise robustness is much cheaper than evaluating  performance. However, due to the conflation, current NQCS methods have to evaluate the intrinsic performance of all candidate circuits, which leads to redundant evaluation costs. 

%     % Further, current NQCS methods conflate the learning ability and noise robustness of candidate circuits by measuring candidate performance on the target device, preventing the effective use of noise information and necessitating performance evaluation for all candidates. Since candidate circuits with low noise robustness will perform badly on the target device regardless of their learning ability, and noise robustness is far cheaper to estimate than circuit performance, performance evaluation for all candidate circuits leads to wasted search time and larger search costs. 
    
%     % Furthermore, current NQCS methods characterize candidate circuit performance by directly measuring performance on the noisy target device, conflating circuit performance and noise robustness. Consequently, circuit performance must be estimated for every candidate circuit regardless of the noise robustness of the circuit. Since estimating circuit performance is far more expensive than estimating circuit noise robustness, this leads to additional unnecessary search overhead.
    
%     % Furthermore, current NQCS methods extend cNAS evalution strategies while accounting for quantum hardware noise by directly measuring candidate circuit performance on the target device. This leads to conflation of a circuit's intrinsic performance and noise robustness, forcing current NQCS methods to estimate circuit performance, which is much costlier than estimating circuit noise robustness alone, for every candidate circuit, resulting in 
    
%     % \item \textbf{Classically-inspired search algorithms are incapable of searching for classical-to-quantum data embeddings:}
%     % Unlike in classical machine learning, the choice of data embedding used for QML tasks is non-trivial. Recent literature ~\cite{schuld2021encodingexpressivity, sweke2021encodingdependentbounds, schuld2022fourierinterpolation} has shown that data embeddings are a key determinant of VQC performance on QML tasks. However, the classically-inspired search algorithms used in current NQCS methods overlook the problem of searching for a data embedding and assume a fixed embedding for every candidate circuit. This design choice precludes the possibility of optimizing the data embedding used based on the specific QML task to be solved, severely limiting model performance. Figure \ref{fig:embeddings} shows the importance of optimizing data embeddings using a simple 1-qubit example.
    
    
%     \item \textbf{Classically-inspired search spaces are device topology agnostic:}  Classical neural network topologies are not constrained by hardware \cite{he2019randomlywired} due to efficient data movement and the high fidelity of classical operations. Thus cNAS methods use topology-agnostic search spaces \cite{hutter2019nb101, yi2020nb201, radosavovic202nds}. Current NQCS methods also follow this design choice \cite{wang2021quantumnas, dacheng2020quantumsupernet}. However, because of the constrained topology of current quantum devices, expensive and error-prone quantum SWAP gates needs to be introduced during circuit compilation for device agnostic circuits. To avoid these additional SWAP gates, current NQCS methods are forced to search for qubit mappings for candidate circuits \cite{wang2021quantumnas}, which introduces additional search overhead. 

    
%     \item \textbf{Classically-inspired search algorithms are incapable of searching for classical-to-quantum data embeddings:} In QML, classical data needs to be non-trivially encoded into a quantum circuit and this process is called \textit{data embedding}. Recent literature ~\cite{schuld2021encodingexpressivity, sweke2021encodingdependentbounds, schuld2022fourierinterpolation} has shown that data embeddings are a key determinant of VQC performance. \cref{fig:embeddings} in \cref{sec:background} shows the importance of data-dependent embeddings using a simple 1-qubit example. Current NQCS methods overlook the problem of optimizing data-embedding and always assume fixed data embedding, which  greatly limit circuit performance.  

% \end{enumerate}

% Current NQCS methods use hardware-agnostic search spaces that do not account for device topology and the error characteristics of individual qubits. As a result, the selected circuits often do not match the topology of the target device, and thus require the insertion of SWAP gates to allow for two-qubit gates between qubits that are not directly connected on the target device. Since SWAP gates are constructed using 3 consecutive CNOT gates, the circuits returned by current NQCS methods often increase significantly in depth due to SWAP gate insertion to match device topology. Since CNOT gate error rates on current NISQ devices are about 1\% \Sash{cite}, the insertion of several SWAP gates can severely impact the fidelity of a circuit, worsening performance on QML tasks.

% In order to minimize the number of SWAP gates required, NQCS methods often utilize an additional search over the space of possible logical-to-physical qubit mappings for a candidate circuit. For example, QuantumNAS \cite{wang2021quantumnas} utilizes an evolutionary algorithm to co-search for a circuit and a qubit mapping. However, these additional search procedures are expensive, and often do not completely eliminate the need for SWAP gate insertions.
% }


==> v1/candidate_eval_strategy.tex <==
\section{Circuit performance evaluation}
\label{sec:metrics_explanations}

 Our calculations indicate that more than 90\% of the total quantum circuit executions for SuperCircuit-based QCS methods are performed in the SuperCircuit training step. This is because computing gradients using the parameter-shift rule requires circuit executions linear in the number of parameters, making training on quantum hardware extremely expensive. Thus, eliminating the initial training phase of QCS is crucial for resource efficiency.

% \framework{} addresses this issue by introducing a novel, cheap-to-compute circuit performance predictor, \textit{\metricone{}}, for resource-efficient candidate circuit evaluation. Compared to training-based evaluation strategies, \metricone{} requires far fewer circuit executions (See~\cref{sec:perf_analysis} for detailed resource requirements), but is as effective a predictor of performance as using trained SuperCircuit weights to evaluate candidate circuits. \cref{fig:correlations} shows the correlations obtained between SuperCircuit predicted losses and $\textrm{Rep}(C)$ with trained circuit performance on the FMNIST-2 task. Additionally, despite its effectiveness, \metricone{} is decoupled from other components in \framework{}, and can be hot-swapped for any other performance predictor.

\framework{} addresses this issue by introducing a novel, cheap-to-compute circuit performance predictor, \textit{\metricone{}}, for resource-efficient candidate circuit evaluation. Compared to training-based evaluation strategies, \metricone{} requires far fewer circuit executions, but is as effective a predictor of performance as using trained SuperCircuit weights to evaluate candidate circuits. \cref{fig:correlations} shows the correlations obtained between SuperCircuit predicted losses and $\textrm{Rep}(C)$ with trained circuit performance on the FMNIST-2 task. Additionally, despite its effectiveness, \metricone{} is decoupled from other components in \framework{}, and can be hot-swapped for any other performance predictor.

In this section, we define \metricone{} and provide some intuition about it. Then we discuss how \metricone{} is computed and demonstrate its correlation with circuit performance. \new{Finally, we discuss how we combine \metrictwo{} and \metricone{} to rank the circuits that remain after the noise-guided circuit elimination process.}

%of remaining circuits after the noise-guided circuit rejection step.


\subsection{Predicting Candidate Circuit Performance Using \MetricOne{}}
% Current methods of estimating performance heavily rely on gradient computation, which is expensive on quantum hardware. As a result, candidate evaluation is extremely expensive, leading to unnecessarily large search overheads. If we can eliminate the need to compute gradients during the candidate evaluation process, the entire NQCS search process can be sped up drastically. To this end, we introduce a gradient-free estimate of candidate circuit performance, which we term \emph{\metricone{}}.

Intuitively, \metricone{} measures the intra-class similarities and inter-class separation of the final quantum states for a variational circuit. As illustrated in~\cref{fig:rep_cap_diag}, the larger the inter-cluster distance and the smaller the intra-cluster distance in the final qubit state space, the higher the \metricone{} of a variational circuit is. A higher \metricone{} indicates that the circuit has a larger ``capacity" for representing the input data, and likely will perform better. 

The \metricone{} of a circuit $C$ is defined as: 
\begin{equation}
    \new{\textrm{Rep}(C) = 1 - \frac{\| R_C - R_{\textrm{ref}}\|^{2}_{2}}{2 \cdot n_{c} \cdot d_{c}^2},}
    \label{eq:repcap}
\end{equation}
\new{where $d_c$ is the number of samples from each class in $\mathcal{X}_{\text{train}}$, $n_c$ is the number of classes in $\mathcal{X}_{\text{train}}$, $||\cdot||$ is the Frobenius norm, and $R_\text{ref}$ is a $d\times d$ reference matrix that captures the ideal circuit behaviour, i.e. $R_\text{ref}(i, j) = 1$ iff $y_i = y_j$ and $R_\text{ref}(i, j) = 0$ otherwise.} $R_C$ is a $d\times d$  matrix that captures pairwise similarities between the representations of data points $x_i$ and $x_j$ created by circuit $C$, with $R_C{(i, j)} \in [0, 1]$. Further details on computing $\textrm{Rep}(C)$ are in Appendix \ref{sec:rep_cap_computation}.

As shown in Appendix \ref{sec:rep_cap_computation}, \new{computing $\text{Rep}(C)$ requires only $n_c \cdot d_c \cdot n_p$ circuit executions, where $n_p$ is the number of parameter initializations we average over. In practice, we take $d_c = 16$, $n_p = 32$, resulting in $512 \cdot n_c$} circuit executions. Then, for $N_C$ circuits, \framework{} requires \new{$512 \cdot N_C \cdot n_c$} circuit executions, regardless of $|\mathcal{X}|$. This is in contrast to \new{SuperCircuit-based methods, which require $2 \cdot t \cdot |\mathcal{X_{\text{train}}}| \cdot \bar{p} + N \cdot |\mathcal{X_{\text{valid}}}|$} circuit executions to \first train a SuperCircuit for $t$ epochs via sampling subcircuits with $\bar{p}$ parameters each on average, and then evaluate the performance of $N$ candidate circuits on a separate validation set $\mathcal{X_{\text{valid}}}$. The initial training overhead of a SuperCircuit \new{scales very poorly, since learning larger and more complex datasets requires longer training times and larger circuits, increasing both $t$ and  $\bar{p}$ with $|\mathcal{X_{\text{train}}}|$.} Thus, the cost of evaluating \metricone{} \new{scales more favourably.} For example, for the 16-parameter Moons task (dataset descriptions provided in \cref{sec:experimental_setup}), \framework{} executes only 44x fewer circuits than QuantumNAS; for the 40-parameter MNIST-4 task, the improvement becomes over 1000x. 
\ignore{
\renewcommand\theadalign{bc}
\renewcommand\theadfont{\bfseries}
\renewcommand\theadgape{\Gape[6pt]}
\renewcommand\cellgape{\Gape[6pt]}
\begin{table*}[h]
  \centering
%\setlength{\tabcolsep}{0.1cm} 
%\renewcommand{\arraystretch}{1.1}
    \begin{tabular}{ | c || c | c | c | c | c | c |}
        \hline
         \textbf{Dataset} & Moons-300 & Bank & Vowel-2 & Vowel-4 & MNIST-4 & FMNIST-4\\ 
         \hline
         \textbf{Spearman R Correlation} & -0.663 & -0.582 & -0.655 & -0.573 & -0.568 & -0.621\\
         \hline
    \end{tabular}
    \caption{The correlations between \metricone{} and trained loss computed for 1000 randomly sampled circuits each.}
    \label{tab:correlations_rep_cap}
\end{table*}
}

Importantly, \metricone{} is \new{highly correlated with circuit performance, as shown in~\cref{fig:rep_cor1}}. On average, \metricone{} shows a Spearman’s correlation of 0.632 with circuit performance, indicating that this metric can be used to effectively predict candidate circuit performance. 

%In contrast,  studies~\cite{li2020random, yu2019evaluating} show that training-based evaluation strategies in SuperNet (the classical counterpart of SuperCircuit) have almost zero correlation with the final training loss.


\begin{hintbox}{\color{white}\textbf{Insight 4: Predict circuit performance without training}}
By analyzing the quantum states created by a circuit for different input data, we can cheaply estimate circuit performance.
\end{hintbox}

\subsection{Final evaluation of remaining circuits}
\label{sec:combining_metrics}

\new{To evaluate the remaining circuits, \framework{} combines the \metrictwo{} and the \metricone{} of each circuit} to accurately predict performance on noisy quantum hardware. \new{The composite score} is computed as:
\begin{equation}
    \text{Score}(C) = \text{CNR}(C)^{i_{\text{noise}}} \times \text{Rep}(C)
\end{equation}
The \new{hyperparameter} $i_{\text{noise}}$ controls the relative importance of $\text{CNR}(C)$. Setting $i_{\text{noise}} = 1$ treats both the noise robustness and performance of $C$ as equally important. For all experiments, we set $i_{\text{noise}} = 0.5$. As the last step, \framework{} returns the circuit with the top composite score.























==> v1/discussion.tex <==
\section{Discussion}
\label{sec:discussion}
\subsection{Related works}
\subsubsection{Quantum Machine Learning}
Several theoretical works have shown the potential for quantum advantage in machine learning tasks such as classification~\cite{nature_communication_2021_power_of_data_qml, abbas2020power} and regression~\cite{schuld2022fourierinterpolation}. Various approaches to QML have been proposed, including formulating variational circuits as kernel methods~\cite{schuld2021qmlmodelsarekernelmethods, havlek2019suplearninginquantumenhancedfeaturespaces, nature_communication_2021_power_of_data_qml, haug2021largescaleqml, glick2021covariantkernels, kubler2021inductivebias, tao2021noisykernels, liu2021robustandrigorousspeedup, canatar2022bandwidthinquantumkernels}, and as quantum neural networks~\cite{Silver_Patel_Tiwari_2022, optic, wang2021roqnn, coles2021overparametrizationinqnns, farhi2018classification, 2019PQC, 2019Expressibility, zoufal2021qbms, nguyen2022equivariantqml, qi2021qtnvqc}. Multiple works~\cite{2019Expressibility, abbas2020power} introduce metrics that aim to measure circuit performance before training, but they are not suitable for QCS due to their high cost.

\subsubsection{QCS for Variational Quantum Algorithms (VQAs)}
A few studies have explored quantum circuit search for VQAs~\cite{vqa_survey}, such as QAOA~\cite{yao2022mctsqaoa}, VQE~\cite{huang2022qceat}, and state preparation~\cite{hong2020dqas, metaqas, continuousQAS}. These works also largely adapt search techniques in classical ML. For example, QCEAT~\cite{huang2022qceat} is similar to evolutionary search-based NAS~\cite{quoc2018evosearchnas}, and MCTS-QAOA~\cite{yao2022mctsqaoa} uses an RL-based candidate sampling mechanism similar to~\cite{baker2016rlnas, quoc2016rlnas}. These frameworks can be extended to perform QCS for QML tasks. However, due to their use of techniques from classical NAS, these methods face the same issues as QCS methods for QML, and are extremely slow even for small QML tasks. We compare \framework{} with \cite{huang2022qceat, yao2022mctsqaoa} in \cref{tab:qcs_comparison}.

\subsubsection{Noise-aware quantum compilation and training}
Recent compilation works explore different levels of circuit transformations to improve noise robustness, including gate cancellation~\cite{xu2022quartz, nam_optimization, efficient_exact_matching}, efficient qubit mapping and routing~\cite{patel2022geyser, lye2015determining, oddi2018greedy, baker2020time, wille2014optimal, nannicini2021optimal, smith2021error, liu2022not, liu2021relaxed, noiseadaptive, tannu2019not}, error mitigation~\cite{jigsaw, adapt, disq, qraft}, circuit synthesis~\cite{patel2022quest, weiden2022topology, patel2022robust, younis2021qfast, peterson2022optimal}, and pulse-level optimizations~\cite{gokhale2020optimized,shi2019optimized, liang2022pan, meirom2022pansatz}. Some of these works~\cite{adapt, das2022imitationgame, ravi2022cliffordcanarycircuits} have used Clifford replicas for characterizing device noise or to create enhanced compilation passes. \framework{}, on the other hand, is the first application of Clifford replicas to QML, and uses them to perform a noise-guided search for QML circuits. Other works focus on increasing noise robustness for QML circuits through improved training procedures~\cite{wang2021quantumnat, wang2022qoc}, an approach complementary to \framework{}, as these techniques can be combined with \framework{} to improve the training of circuits selected by \framework{}.

% \subsubsection{QCS for Variational Quantum Algorithms (VQAs)}
% \new{A few studies have explored quantum circuit search for VQAs~\cite{vqa_survey}, such as QAOA~\cite{yao2022mctsqaoa}, VQE~\cite{huang2022qceat}, and state preparation~\cite{hong2020dqas, metaqas, continuousQAS}. These works also largely adapt search techniques in classical ML. For example, QCEAT~\cite{huang2022qceat} is similar to evolutionary search-based NAS~\cite{quoc2018evosearchnas}, and MCTS-QAOA~\cite{yao2022mctsqaoa} uses an RL-based candidate sampling mechanism similar to~\cite{baker2016rlnas, quoc2016rlnas}.}

% \subsubsection{QCS for QML} Currently, the leading QCS methods for QML include QuantumNAS~\cite{wang2021quantumnas} and QuantumSupernet~\cite{dacheng2020quantumsupernet}, which we compare with \framework{} in~\cref{sec:evaluation}. These methods share very similar designs inherited from the supernet formalism in classical ML~\cite{dean2018classicalsupernet, pham2018enas}. 

\subsection{Comparison with prior works on data embeddings}
Several works \cite{schuld2021encodingexpressivity, schuld2022fourierinterpolation, sweke2021encodingdependentbounds} have investigated the effect of data embeddings on circuit performance through the lens of generalization bounds and Fourier series. These works target a problem aim to shed light on the behavioural properties of QML circuits, and thus focus on simplified theroretical settings. In contrast, \framework{} aims to search for a performant and noise-robust circuit for a given QML task and target device, which is a fundamentally different problem.

\subsection{Comparison with prior QCS works for QML}
 A few studies have focused on QCS for QML tasks, such as QuantumNAS~\cite{wang2021quantumnas} and QuantumSupernet~\cite{dacheng2020quantumsupernet}. These methods are both based on the classical Supernet \cite{dean2018classicalsupernet, pham2018enas} framework, and are very similar. QuantumNAS has been extensively discussed in \cref{sec:intro}, and compared with \framework{} in \cref{sec:evaluation}. \framework{} abandons the SuperCircuit framework, and thus avoids the numerous drawbacks associated with its classically-inspired design. Instead, \framework{} adopts a novel QCS pipeline that generates device-aware circuits, decouples circuit noise robustness and performance evaluation, and uses gradient-free performance predictors. In~\cref{tab:qcs_comparison}, we present a summary of the differences between \framework{} and other QCS methods for QML.

\renewcommand\theadalign{bc}
\renewcommand\theadfont{\bfseries}
\renewcommand\theadgape{\Gape[6pt]}
\renewcommand\cellgape{\Gape[6pt]}
\renewcommand{\arraystretch}{1.2}
\begin{table*}[t]
    \centering
    \setlength{\tabcolsep}{0.22cm}
    \caption{\imp{Key differences between \framework{} and existing QCS methods.}}
    \begin{tabular}{l c c c c c c }
        \toprule
       \imp{Framework} & \makecell{\imp{Search}\\\imp{Space}} & \makecell{\imp{Search}\\\imp{Algorithm}} & \makecell{\imp{Candidate}\\\imp{Evaluation Strategy}} & \makecell{\imp{\framework{}}\\\imp{Speedup}} & \makecell{\imp{Runtime}\\\imp{Bottleneck}}\\
        %\hline
        \midrule
        \imp{QCEAT~\cite{huang2022qceat}} & \makecell{\imp{Device-agnostic}\\\imp{random circuits}} & \makecell{\imp{Evolutionary}\\\imp{search}} & \makecell{\imp{Train}\\\imp{circuit}} & \makecell{\imp{9403$\times$}} & \makecell{\imp{Gradient}\\\imp{computation}}\\
        
        \imp{MCTS-QAOA~\cite{yao2022mctsqaoa}} & \makecell{\imp{Device-agnostic}\\\imp{Pauli strings}} & \makecell{\imp{RL + MCTS}} & \makecell{\imp{Train}\\\imp{circuit}} & \makecell{\imp{9856$\times$}} & \makecell{\imp{Uses RL}\\\imp{(sample inefficient)}}\\
        
        \imp{QuantumSupernet~\cite{dacheng2020quantumsupernet}} & \makecell{\imp{Device-agnostic}\\\imp{SuperCircuit}} & \makecell{\imp{Random}\\\imp{search}} & \makecell{\imp{SuperCircuit}\\\imp{predicted loss}} & \makecell{\imp{349$\times$}} & \makecell{\imp{Gradient}\\\imp{computation}}\\
        
        \imp{QuantumNAS~\cite{wang2021quantumnas}} & \makecell{\imp{Device-agnostic}\\\imp{SuperCircuit}} & \makecell{\imp{Evolutionary}\\\imp{search}} & \makecell{\imp{SuperCircuit}\\\imp{predicted loss}} & \makecell{\imp{185.6$\times$}} & \makecell{\imp{Gradient}\\\imp{computation}}\\
        
        \midrule
        \textbf{\imp{\framework{}}} & \makecell{\imp{\textbf{Device- and noise-}}\\\imp{\textbf{aware circuits}}} & \makecell{\imp{\textbf{Noise-guided}}\\\imp{\textbf{random search}}} & \makecell{ \imp{\textbf{\MT{} and}}\\ \imp{\textbf{\MO{}}}} & \makecell{\imp{--}} & \makecell{\imp{--}}\\
        \bottomrule
        \end{tabular}
    \label{tab:qcs_comparison}
    % \vspace*{-0.4cm}
\end{table*}

\subsection{\imp{Limitations of SuperCircuit-based methods}}
It is tempting to try to incorporate \framework{}'s improvements into SuperCircuit-based methods to close the gap between them and \framework{} both in terms of resource efficiency and performance. However, this is not feasible, as SuperCircuit-based methods are fundamentally incompatible with many of \framework{}'s key contributions. We illustrate this here using QuantumNAS~\cite{wang2021quantumnas} as an example.

\begin{enumerate}[leftmargin=0cm,itemindent=.5cm,labelwidth=\itemindent,labelsep=0cm,align=left, itemsep=0.2cm, listparindent=0.4cm]
    \item \textbf{Device-aware circuit generation}: A key design decision made by QuantumNAS~\cite{wang2021quantumnas} is to share one topology-agnostic SuperCircuit across multiple quantum devices due to the high cost of SuperCircuit training, which precludes the possibility of using a device-aware SuperCircuit. 
    
    \item \textbf{Searching for data embeddings}: A key limitation of SuperCircuits is the inability to reliably predict candidate circuit performance when candidate circuits use different data embeddings. Thus, QuantumNAS cannot search for data embeddings while predicting circuit performance accurately.
    
    \item \textbf{Cheaply rejecting low-fidelity circuits}: QuantumNAS must perform SuperCircuit training before the circuit-mapping evolutionary co-search, preventing it from identifying and cheaply rejecting low-fidelity circuits.
    
    \item \textbf{Using gradient-free performance predictors}: Performing circuit performance evaluation without computing gradients is impossible for QuantumNAS as their circuit performance prediction requires a trained SuperCircuit.
\end{enumerate}

% \renewcommand\theadalign{bc}
% \renewcommand\theadfont{\bfseries}
% \renewcommand\theadgape{\Gape[6pt]}
% \renewcommand\cellgape{\Gape[6pt]}
% \renewcommand{\arraystretch}{1.2}
% \begin{table*}[t]
%     \centering
%     \setlength{\tabcolsep}{0.05cm}
%     \begin{tabular}{l c c c c c c }
%         \toprule
%        \imp{Framework} & \makecell{\imp{Search}\\\imp{Space}} & \makecell{\imp{Search}\\\imp{Algorithm}} & \makecell{\imp{Candidate}\\\imp{Evaluation}\\\imp{Strategy}} & \makecell{\imp{Circuit Executions}\\\imp{Required}} & \makecell{\imp{Elivagar}\\\imp{Speedup}\\\imp{(GMean)}} & \makecell{\imp{Runtime}\\\imp{Bottleneck}}\\
%         %\hline
%         \midrule
%         \imp{QCEAT~\cite{huang2022qceat}} & \makecell{\imp{Device-agnostic}\\\imp{random circuits}} & \makecell{\imp{Evolutionary}\\\imp{search}} & \makecell{\imp{Train}\\\imp{circuit}} & \makecell{\imp{$N_{outer} \cdot n_r \cdot t \cdot 2 \cdot \bar{p} \cdot$}\\\imp{ $|\mathcal{X}_{train}| \cdot \left [ 5 \cdot 2^{N_{inner}} - 4 \right ]$}} & \makecell{\imp{9403$\times$}} & \makecell{\imp{Gradient}\\\imp{computation}}\\
%         \imp{MCTS-QAOA~\cite{yao2022mctsqaoa}} & \makecell{\imp{Device-agnostic}\\\imp{Pauli strings}} & \makecell{\imp{RL + MCTS}} & \makecell{\imp{Train}\\\imp{circuit}} & \makecell{\imp{$T_{iter} \cdot T_{init} \cdot$} \\ \imp{$[ R \cdot t \cdot |\mathcal{X}_{train}| + |\mathcal{X}_{valid}| ]$}} & \makecell{\imp{9856$\times$}} & \makecell{\imp{Uses RL}\\\imp{(extremely sample} \\\imp{inefficient)}}\\
%         \imp{QuantumSupernet~\cite{dacheng2020quantumsupernet}} & \makecell{\imp{Device-agnostic}\\\imp{SuperCircuit}} & \makecell{\imp{Random}\\\imp{search}} & \makecell{\imp{Run subcircuit}\\\imp{with SuperCircuit}\\\imp{params}} & \makecell{\imp{$t \cdot 2 \cdot \bar{p} \cdot |\mathcal{X}_{train}| +$}\\ \imp{$|\mathcal{X}_{valid}| \cdot N_C$}} & \makecell{\imp{349$\times$}} & \makecell{\imp{Gradient}\\\imp{computation}}\\
%         \imp{QuantumNAS~\cite{wang2021quantumnas}} & \makecell{\imp{Device-agnostic}\\\imp{SuperCircuit}} & \makecell{\imp{Evolutionary}\\\imp{search}} & \makecell{\imp{Run subcircuit}\\\imp{with SuperCircuit}\\\imp{params}} & \makecell{\imp{$t \cdot 2 \cdot \bar{p} \cdot |\mathcal{X}_{train}| +$}\\ \imp{$|\mathcal{X}_{valid}| \cdot N_C$}} & \makecell{\imp{185.6$\times$}} & \makecell{\imp{Gradient}\\\imp{computation}}\\
%         \midrule
%         \textbf{\imp{\framework{}}} & \makecell{\imp{\textbf{Device- and}}\\\imp{\textbf{noise-aware circuits}}} & \makecell{\imp{\textbf{Noise-guided}}\\\imp{\textbf{random}} \\ \imp{\textbf{search}}} & \makecell{ \imp{\textbf{CNR and}}\\ \imp{\textbf{Rep(C)}}} & \makecell{ \imp{\textbf{$O(N_C \cdot n_c)$}}} & \makecell{\imp{--}} & \makecell{\imp{--}}\\
%         \bottomrule
%         \end{tabular}
%     \caption{\imp{Summary of \framework{} and existing QCS methods.}}
%     \label{tab:qcs_comparison}
%     % \vspace*{-0.4cm}
% \end{table*}

% \renewcommand\theadalign{bc}
% \renewcommand\theadfont{\bfseries}
% \renewcommand\theadgape{\Gape[6pt]}
% \renewcommand\cellgape{\Gape[6pt]}
% \renewcommand{\arraystretch}{1.2}
% \begin{table*}[t]
%     \centering
%     \setlength{\tabcolsep}{0.05cm}
%     \begin{tabular}{l c c c c c c }
%         \toprule
%        \imp{Framework} & \makecell{\imp{Search}\\\imp{Space}} & \makecell{\imp{Search}\\\imp{Algorithm}} & \makecell{\imp{Candidate}\\\imp{Evaluation}\\\imp{Strategy}} & \makecell{\imp{Circuit Executions}\\\imp{Required}} & \makecell{\imp{Elivagar}\\\imp{Speedup}\\\imp{(GMean)}} & \makecell{\imp{Runtime}\\\imp{Bottleneck}}\\
%         %\hline
%         \midrule
%         \imp{QCEAT~\cite{huang2022qceat}} & \makecell{\imp{Device-agnostic}\\\imp{random circuits}} & \makecell{\imp{Evolutionary}\\\imp{search}} & \makecell{\imp{Train}\\\imp{circuit}} & \makecell{\imp{$N_{outer} \cdot n_r \cdot t \cdot 2 \cdot \bar{p} \cdot$}\\\imp{ $|\mathcal{X}_{train}| \cdot \left [ 5 \cdot 2^{N_{inner}} - 4 \right ]$}} & \makecell{\imp{9403$\times$}} & \makecell{\imp{Gradient}\\\imp{computation}}\\
%         \imp{MCTS-QAOA~\cite{yao2022mctsqaoa}} & \makecell{\imp{Device-agnostic}\\\imp{Pauli strings}} & \makecell{\imp{RL + MCTS}} & \makecell{\imp{Train}\\\imp{circuit}} & \makecell{\imp{$T_{iter} \cdot T_{init} \cdot$} \\ \imp{$[ R \cdot t \cdot |\mathcal{X}_{train}| + |\mathcal{X}_{valid}| ]$}} & \makecell{\imp{9856$\times$}} & \makecell{\imp{Uses RL}\\\imp{(extremely sample} \\\imp{inefficient)}}\\
%         \imp{QuantumSupernet~\cite{dacheng2020quantumsupernet}} & \makecell{\imp{Device-agnostic}\\\imp{SuperCircuit}} & \makecell{\imp{Random}\\\imp{search}} & \makecell{\imp{Run subcircuit}\\\imp{with SuperCircuit}\\\imp{params}} & \makecell{\imp{$t \cdot 2 \cdot \bar{p} \cdot |\mathcal{X}_{train}| +$}\\ \imp{$|\mathcal{X}_{valid}| \cdot N_C$}} & \makecell{\imp{349$\times$}} & \makecell{\imp{Gradient}\\\imp{computation}}\\
%         \imp{QuantumNAS~\cite{wang2021quantumnas}} & \makecell{\imp{Device-agnostic}\\\imp{SuperCircuit}} & \makecell{\imp{Evolutionary}\\\imp{search}} & \makecell{\imp{Run subcircuit}\\\imp{with SuperCircuit}\\\imp{params}} & \makecell{\imp{$t \cdot 2 \cdot \bar{p} \cdot |\mathcal{X}_{train}| +$}\\ \imp{$|\mathcal{X}_{valid}| \cdot N_C$}} & \makecell{\imp{185.6$\times$}} & \makecell{\imp{Gradient}\\\imp{computation}}\\
%         \midrule
%         \textbf{\imp{\framework{}}} & \makecell{\imp{\textbf{Device- and}}\\\imp{\textbf{noise-aware circuits}}} & \makecell{\imp{\textbf{Noise-guided}}\\\imp{\textbf{random}} \\ \imp{\textbf{search}}} & \makecell{ \imp{\textbf{CNR and}}\\ \imp{\textbf{Rep(C)}}} & \makecell{ \imp{\textbf{$O(N_C \cdot n_c)$}}} & \makecell{\imp{--}} & \makecell{\imp{--}}\\
%         \bottomrule
%         \end{tabular}
%     \caption{\imp{Summary of \framework{} and existing QCS methods.}}
%     \label{tab:qcs_comparison}
%     % \vspace*{-0.4cm}
% \end{table*}





==> v1/experimental_methodology.tex <==

\section{Experimental Setup}
\label{sec:experimental_setup}

\subsection{Benchmarks}

We conduct experiments on 8 different QML benchmarks. A summary of the datasets used is shown in~\cref{tab:datasets}. \new{Num. Param.} in~\cref{tab:datasets} refers to the number of parameters in the circuits we search for in \cref{sec:evaluation}. We center-crop the original 28x28 images to 24x24 and downsample to 4x4 for all MNIST and FMNIST dataset variants. The Vowel-2 dataset is constructed by merging 8 out of the 9 classes in the original dataset into 2 classes. The Vowel-4 dataset uses the same 8 classes, but merged into 4 classes instead of 2. We sample a subset of the original Bank dataset in order to obtain a balanced dataset from the original unbalanced data. The \new{Moons} dataset is a synthetically generated 2-class, 2-dimensional dataset constructed using the scikit-learn package.

\renewcommand\theadalign{bc}
\renewcommand\theadfont{\bfseries}
\renewcommand\theadgape{\Gape[6pt]}
\renewcommand\cellgape{\Gape[6pt]}
\begin{table}[h]
\vspace{-0.05in}
    \caption{Summary of the 8 QML tasks for benchmarking.}
  \centering
\setlength{\tabcolsep}{0.05cm} 
\renewcommand{\arraystretch}{1.2}
    \begin{tabular}{ l  c  c  c  c}
        \toprule
         Benchmark & Classes & Data Dim. & Num. Samples & Num. Param.\\
         \midrule
         Moons & 2 & 2 & 0.60K & 16\\
         Bank & 2 & 4 & 1.22K & 20\\ 
         MNIST-2 & 2 & 4x4 & 2K & 20\\
         MNIST-4 & 4 & 4x4 & 10K & 40\\
         FMNIST-2 & 2 & 4x4 & 2K & 32\\
         FMNIST-4 & 4 & 4x4 & 10K & 24\\
         Vowel-2 & 2 & 10 & 0.72K & 32\\
         Vowel-4 & 4 & 10 & 0.72K & 40\\ 
         \bottomrule
    \end{tabular}
    \label{tab:datasets}
    % \vspace*{-0.4cm}
\end{table}

\subsection{Backends and Compiler Configurations} 

We perform all training and computation of \metricone{} on noiseless simulators using Pennylane~\cite{bergholm2018pennylane} and TorchQuantum~\cite{wang2021quantumnas}. \new{We use 4 real devices (IBMQ-Kolkata, IBMQ-Guadalupe, IBMQ-Mumbai, and IBM-Geneva), and 8 different device noise simulators based on OQC Lucy, Rigetti Aspen-M-2, and 6 IBM devices (IBMQ-Lima, IBMQ-Belem, IBMQ-Quito, IBMQ-Manila, IBM-Nairobi, and IBM-Oslo) to compute \metrictwo{}} and perform inference using trained circuits. \imp{\new{For all competing methods, we use the default Qiskit compiler with optimization level set to 3, except for QuantumNAS, for which we use level 2. We turn off the circuit mapping passes and use optimization level 0 for \framework{} since it generates circuits that do not need mapping.}}

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.93\textwidth]{figs/results/main_braket_v2.png}
    \caption{\imp{Relative circuit performance on the 8 datasets, run on noise models of Rigetti Aspen-M-2, OQC Lucy, IBM-Nairobi, and IBMQ-Manila. The test set MSE loss of the human designed baseline is given below task labels.}}
    \label{fig:main_results}
    % \vspace*{-0.5cm}
\end{figure*}

\subsection{Competing methods}

We compare \framework{} to four competing methods:

\textbf{Random:} we randomly generate topology-unaware circuits that use the same number of qubits and parameters as all the other circuits compared. We generate circuits from two search spaces taken from the QuantumNAS paper, \new{RXYZ + CZ, and RZX + RXX}. \new{We generate 25 circuits, train all of them, and report the average performance.}

\textbf{Human designed (baseline):} We use three data embedding schemes (angle, amplitude, and IQP embedding) paired with stacked layers of alternating RX, RY, RZ, and CX gates using ring connectivity, where every qubit $q_i$ is connected with $q_{i + 1}$ via a CX gate, and the last qubit is connected to the first qubit. We train all three circuits and report the average performance. 

\textbf{QuantumSupernet:} We modify the SuperCircuit training procedure proposed in~\cite{dacheng2020quantumsupernet} by replacing full-batch gradient descent with mini-batch gradient descent with batch size 32 to ensure that all SuperCircuit parameters are updated sufficiently. We train the SuperCircuit for 400 epochs with vanilla SGD using a learning rate of 0.05. We did not perform experiments using QuantumSupernet for all the datasets considered due to the extremely long runtime requirements of the scripts provided in~\cite{dacheng2020quantumsupernet}.
%.as well as the low relative performance of the method.
%We then sample 100 subcircuits, perform evaluation using trained SuperCircuit parameters, select the best subcircuit, and retrain it from scratch.

\textbf{QuantumNAS:} We use the same hyperparameters used for SuperCircuit training and evolutionary search in the original paper~\cite{wang2021quantumnas}. The SuperCircuit is trained for 200 epochs with batch size 32 using the Adam optimizer with an initial learning rate of $5e-3$ with cosine annealing. The evolutionary search is performed for 40 iterations, using a initial population of size 40, parent size 10, crossover population 10, mutation population 20, and mutation probability 0.4. \new{We use two gate sets (RXYZ + CZ and RX + RXX) out of the 6 proposed in~\cite{wang2021quantumnas}}. We find that the evolutionary search process converges to similarly performant subcircuits over multiple random population initializations, and so report the trained performance of the subcircuit returned by one evolutionary search as the performance of QuantumNAS. We do not perform iterative pruning, choosing to train the best subcircuit obtained by the evolutionary search process directly, as the pruning phase does not contribute towards circuit search. 

\subsection{Hyperparameters for \framework{}}
\label{sec:elivagar-hyperparams}
We randomly sample \new{$d_c = 16$ data points from each class of $\mathcal{X}_{\textrm{train}}$ and $n_p = 32$ random parameter initializations to compute the \metricone{}. We use $M = 32$ Clifford replicas to compute \metrictwo{}}. We reject circuits with \metrictwo{} values less than 0.7 or outside the top 50\% of \new{all scores (see~\cref{sec:clifford_noise}). To mitigate the effects} of random circuit sampling, we repeat our workflow 25 times, and report the average performance.  
%We first sample a set of 100 circuit using our device-aware circuit sampling policy, and then compute \metrictwo{} for each circuit. We then eliminate the circuits for which the \metrictwo{} scores are in the bottom half of the set of \metrictwo{} scores. We then compute \metricone{} for the remaining 50 circuits, and then use both \metrictwo{} and \metricone{} to compute composite scores $\text{Score}(C)$ for the circuits via the process outlined in~\cref{sec:combining_metrics}. Finally, we select the circuit with the best $\text{Score}(C)$, and train it from scratch. 

% \subsection{Evaluation metrics}
% We use the mean squared error (MSE) loss incurred by a circuit $C$ on a held-out test portion of a dataset after training as a measure of circuit performance. We report the \emph{relative performance} of the circuits we train 

\subsection{Figure of merit}
We measure the performance of a circuit $C$ using the standard Mean Squared Error over the test portion of a QML task which was not seen during circuit training. For convenience we report performance of circuits relative to a human-designed baseline in \cref{fig:main_results}, given by

\begin{equation}
    \textrm{Perf}_{\textrm{rel}}(C) = \frac{\textrm{MSE}(C_{\textrm{baselines}})}{\textrm{MSE}(C)}
\end{equation}

==> v1/introduction.tex <==

\section{Introduction}
\label{sec:intro}
%Quantum computing has reached an inflection point where there is growing impetus to use them for solving real-world problems. However, noisy quantum devices lead to computational errors that result in poor application fidelity. As quantum programs are executed on  systems in the presence of errors, the fidelity of applications must be improved.%To run practical quantum applications, their fidelity must be improved. 
%In the \textit{Noisy-Intermediate Scale Quantum (NISQ)} era~\cite{Preskill2018quantumcomputingin}, quantum computers execute programs in the presence of errors and require quantum algorithms to reconcile with device noise.
  
% In NISQ-era~\cite{Preskill2018quantumcomputingin}, 

Quantum Machine Learning (QML) is an important class of quantum algorithms for the \textit{Noisy-Intermediate Scale Quantum (NISQ)}~\cite{Preskill2018quantumcomputingin} era, due to its applicability to real-world problems such as classification \cite{wang2021quantumnas, farhi2018classification, lloyd2020quantum, nature_communication_2021_power_of_data_qml}, generative modeling \cite{huang2021qgans, neven2021entanglingqgans, ortiz2020iontrapqgans, zoufal2021qbms, zoufal2021thesis} and learning physical systems \cite{nature_2021_rigorous_speedup_qml, huang2022advantagefromexperiments}. QML uses \textit{variational} quantum circuits as the underlying model to perform machine learning tasks. The parameters in these variational circuits are iteratively updated (i.e., \textit{trained}) using a classical optimizer until the circuit learns the input problem to high accuracy. 

The key challenge in designing effective near-term QML algorithms is to find variational circuits with good \textit{circuit performance} (i.e., learning ability) and \textit{noise robustness}. Variational circuits must be performant to accurately learn the input problem, and be noise robust to avoid performance degradation. However, due to the complexity of device-level noise sources and the nascent state of QML theory, there are few established guiding principles in designing QML circuits. Current manually crafted circuits are often under-performant, and face numerous practical issues such as vanishing gradients~\cite{wang2021noiseinduced} and low fidelity.

\begin{figure}[t]
        \centering
        \includegraphics[width=0.75\columnwidth]{figs/introduction/classical vs quantum@3x.png}
        
        \caption{Comparison of Classical and Quantum ML systems.}
        \vspace*{-0.4cm}
        \label{fig:ml_comparison}
    \end{figure}

%Because that the classical optimizations are often intrinsically stochastic, this classical-quantum hybrid training process is relatively noise tolerant, making QML algorithms suitable for the current Noisy-Intermediate Scale Quantum (NISQ) devices.


%Under this classical-quantum hybrid framework, there is a vast design space to improve the learning ability and noise robustness of QML algorithms.


%Due to the similarity of the underlying problem, QCS methods can be characterized by the decomposition \cite{elsken2018nassurvey} proposed for classical Neural Architecture Search (cNAS) ~\cite{li2019nassurvey, ning2020classicalnassurvey}  ---   \textbf{candidate evaluation strategy}, \textbf{search algorithm} and  \textbf{search space}, with one difference: the candidate evaluation strategy of QCS methods must not only estimate the \emph{intrinsic performance} of candidate circuits (circuit performance on a noiseless device), but also their \emph{noise robustness} on real quantum hardware.

%, and using QuantumNAS \cite{wang2021quantumnas} for the MNIST-4 classification task results in a search cost of about $1.4 \cdot 10^8$ circuit evaluations, while only slightly outperforming commonly used human-designed VQCs (see \cref{sec:evaluation}

This challenge has motivated recent efforts in \textbf{Quantum Circuit Search (QCS)}~\cite{wang2021quantumnas, dacheng2020quantumsupernet, hong2020dqas} which aim to automatically search for high-performance noise-robust variational circuits. While promising, these methods are still preliminary and naively adopt established methodologies from classical Neural Architecture Search (NAS)~\cite{li2019nassurvey, ning2020classicalnassurvey}, a subfield of Machine Learning (ML) that searches for high-performance neural networks. Consequently, current QCS works overlook the fundamental differences between classical ML and QML, as shown in~\cref{fig:ml_comparison}. %, QML and classical ML systems are  different at all levels. 
 At the data processing level, classical ML uses multi-dimensional vectors to represent input data. In QML, each data dimension must be embedded into \textit{data embedding} gates, and the choices and locations of these gates directly impact circuit performance. At the algorithm level, QML cannot perform gradient computation efficiently via automatic differentiation as intermediate qubit states cannot be copied~\cite{nocloning} and collapse upon measurement~\cite{NielsenChuang}. Instead, it requires methods like parameter-shift rules~\cite{schuld2019analyticgradients} that scale poorly with problem sizes. At the compilation level, mapping classical neural networks with arbitrary topology onto memory incurs little cost because of efficient data movement. However, in QML, due to the limited connectivity of NISQ devices, there is a huge routing cost introduced by the insertion of error-prone SWAP gates when the circuit does not match the device topology. 
 
\begin{figure}[t]
        \centering
        \includegraphics[width=0.7\columnwidth]{figs/introduction/qNAS@3x.png}
        
        \caption{QuantumNAS: A state-of-the-art QCS framework.}
        \vspace*{-0.2cm}
        \label{fig:quantumnas}
\end{figure}
    
Existing QCS methods naively adapt classical ML designs and therefore are incompatible with the unique constraints of QML. We explain these mismatches using QuantumNAS~\cite{wang2021quantumnas}, a state-of-the-art QCS method. As shown in ~\cref{fig:quantumnas}, QuantumNAS first 
trains a large topology-agnostic ``SuperCircuit" with a fixed data embedding. Next, it performs an evolutionary co-search to identify a performant and noise-robust circuit-qubit mapping pair, using the trained parameters of the SuperCircuit to evaluate the performance of candidate circuits on the target NISQ device. Finally, QuantumNAS returns the best circuit found by the evolutionary search process. Other competitive QCS frameworks, such as QuantumSupernet~\cite{dacheng2020quantumsupernet}, also follow similar designs, and thus all experience the following issues:

\begin{enumerate}[leftmargin=0cm,itemindent=.5cm,labelwidth=\itemindent,labelsep=0cm,align=left, itemsep=0.2cm, listparindent=0.4cm]
    %\item Classically-inspired search spaces are device-topology agnostic, leading to additional circuit-mapping co-search costs and hardware-inefficient circuits that require SWAP gate insertion.
    \item Their use of device topology agnostic search spaces result in additional search costs for logical-to-physical qubit mappings. Moreover, these mappings are still hardware-inefficient, since the searched circuits usually do not match the device topology and quantum SWAP gates must be inserted before circuit execution on real hardware.

    %\item Classically-inspired search strategies overlook the importance of data embeddings and use fixed, dataset-agnostic data embeddings, which severely bottlenecks circuit performance.
    \item They do not assess the impact of data embeddings on circuit performance as they use fixed, dataset-agnostic data embeddings. This leads to circuits with poor performance.

    %\item Classically-inspired performance evaluation strategies heavily rely on training, thus, gradient computation, which are expensive on quantum computers and scale poorly with circuit size. 
    \item They adopt training-based performance evaluation strategies from classical ML that heavily rely on gradient computation. These evaluation strategies are expensive on quantum computers and scale poorly with circuit and dataset size. 
    
    %\item Classically-inspired evaluation strategies measure circuit performance directly on the target device, conflating the cheap evaluation of circuit noise robustness and the expensive evaluation of circuit performance, preventing early rejection of low-fidelity circuits and leading to unnecessary search costs.
    \item They perform expensive performance evaluation for all circuits, which leads to unnecessary overheads, since many circuits have extremely low fidelity. These circuits will perform poorly regardless of learning ability due to the severe corruption of circuit outputs by device noise. Existing methods do not have any mechanisms to identify and eliminate the expensive performance evaluation for such circuits. 
\end{enumerate}

\begin{figure*}[t]
    \centering

     \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/background/SWAP@3x.png}
         \caption{}
         \label{fig:swap}
     \end{subfigure}
\hfill
     \begin{subfigure}{0.35\textwidth}
     \centering      \includegraphics[width=\textwidth]{figs/background/circs@3x.png}    \includegraphics[width=\textwidth]{figs/background/3c@3x.png}
      \caption{}
      \label{fig:embedding}
     \end{subfigure}
\hfill
     \begin{subfigure}[b]{0.35\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/background/QML@3x.png}
         \caption{}
         \label{fig:qml}
     \end{subfigure} 
\hfill  
 
    \caption{(a) Circuit and device topology mismatch \new{results in a} large routing cost due to expensive and error-prone SWAP gates. (b) Both circuits use the same trainable gates, but different data embeddings. \new{Circuit 2 fails to learn the target function but Circuit 1 succeeds, highlighting the importance of using a suitable data embedding for QML tasks.} (c) Training in QML involves iterations between a variational circuit and a classical optimizer. } % The circuit returns the gradients of circuit parameters and the classical optimizer use them to guide the parameter updates in the next iteration %% Circuit 1 and 2 share the same variational part of the circuit ($U_3(\vec{\theta_1})$, $U_3(\vec{\theta_2})$ gates) but have different data embeddings ($\{R_x(x), R_y(x)\}$ vs $R_x(x)$), circuit 1 can correctly learn the input function  \( f(x) = -0.75\sin{2x} + 0.05\) but circuit 2 fails
     
    % \vspace*{-0.4cm}
    \label{fig:background}
\end{figure*}

Consequently, existing QCS frameworks incur significant search overheads even for small circuits and problem sizes. For example, to design a 4-qubit, 24-parameter circuit for the FMNIST-4 classification task, QuantumNAS requires executing more than $10^{8}$ quantum circuits, requiring more than 3 years on the fastest superconducting quantum computers.

To address the problems above, we propose \framework{}, a resource-efficient, high-performance QCS framework tailored to QML systems. \textbf{First}, \framework{} performs a noise-guided search \new{based on target device} topology to generate noise robust circuits that require no SWAP gate insertions. This strategy not only ensures the hardware-efficiency of generated circuits but also eliminates the costly circuit-mapping co-search (issue 1). \textbf{Second}, to mitigate the performance bottlenecks in current QCS frameworks caused by fixed, data-agnostic data embeddings (issue 2), \framework{} \new{randomly samples a subset of the gates in candidate circuits to use as data embedding gates, allowing \framework{} to search for the optimal data embedding for a QML task.}
\textbf{Third}, to reduce the overheads of training-based circuit evaluations (issue 3), \framework{} introduces a novel, cheap-to-compute performance predictor, \textit{\metricone{}}, for circuit performance evaluation. By leveraging this predictor, \framework{} eliminates the expensive training step in the QCS workflow while retaining the ability to effectively predict circuit performance. \textbf{Last}, \framework{} makes use of the insight that evaluating noise robustness is much simpler than performance evaluation. By introducing \textit{\metrictwo{}}, a predictor of noise robustness, it  decouples these two evaluations to enable early rejection of low-fidelity circuits (issue 4). \metrictwo{} takes advantage of the fact that the noise robustness of circuits can be accurately predicted by analyzing their Clifford replicas, which can be efficiently simulated on classical computers~\cite{PhysRevLett_cliffordSimulation}. \new{By comparing the outputs of a few Clifford replicas of a circuit run on noisy quantum hardware and a noiseless simulator, \framework{} can cheaply detect and eliminate low-fidelity circuits early in the search process.}

%We conduct experiments on 8 different QML benchmarks to evaluate \framework{}. Compared to current QCS methods, \framework{} finds circuits with 10\% better performance on average while requiring only 0.3\% of  quantum circuit executions (i.e., 313x faster and more resource efficient). Importantly, we show that the resource-efficiency and speedup of \framework{} over current QCS methods increases with the input problem size.

Our evaluations using 8 near-term QML benchmarks show that \framework{} finds circuits with \perfgain{} higher accuracy on average while being \speedup{} faster and more resource efficient that prior state-of-the-art QCS methods. Moreover, we show that the efficiency advantage of \framework{} increases with problem size.


%For example, we use an analytical model to estimate the performance the speedup for \framework{} to search for a 100-parameter circuit for a 60000-sample MNIST-10 dataset, which suggests the speedup to be 8629x over QuantumNAS. In comparison, this is much larger than the 646x speedup we obtained from our largest experiments for searching for 24-parameter circuit for the 8000-sample FMNIST-4 dataset.




In summary, the contributions of this paper are:
\begin{enumerate}[leftmargin=0cm,itemindent=.5cm,labelwidth=\itemindent,labelsep=0cm,align=left, itemsep=0.2cm, listparindent=0.4cm]
    \item  We propose a novel QCS workflow, \framework{}, that is tailored to QML systems and addresses the design flaws in current classically-inspired QCS methods. 
    
    \item We show that noise-guided, topology-aware and data embedding-aware circuit search, on average, leads to a \perfgain{} improvement in circuit performance compared to current methods.

    \item We show that by using \metricone{} to predict circuit performance, the number of circuit executions in \framework{} can be improved by 22$\times$- 523$\times$ relative to training-based evaluation strategies.

    \item We show that by performing early rejection of low-fidelity circuits using \metrictwo{}, the resource efficiency of \framework{} can be further improved by 2$\times$-20$\times$ depending on noise level.

    
    %\item We propose to co-search for the data embedding and the variational circuits of candidate circuits for the first time. We show that this search strategy improves the performance of resulting circuits by \TD{10\%}.
    
    % \item With a comprehensive evaluation on 8 QML benchmarks on real quantum devices and noise simulators, we demonstrate that \framework{} outperforms current QCS methods by 10\% on average, while using 0.3\% resources.
\end{enumerate}

We open source \framework{} to facilitate future QCS research: \url{https://anonymous.4open.science/r/Elivagar-8BB0}.



==> v1/performance_analysis.tex <==
\section{Performance Analysis}
\label{sec:perf_analysis}

% just headings to remind me what to add
\subsection{Device-aware circuit generation}
\label{sec:device_aware_gen}

\imp{To analyze the effect of \new{\framework{}'s circuit generation} versus na\"ive random circuit generation, \new{we compare device-aware circuits generated via \framework{} with randomly generated, device-unaware circuits} on multiple devices. \new{We generate pairs of device-aware and -unaware circuits with the same number of 1- and 2-qubit gates before compilation in order to ensure a fair comparison, and show the average characteristics in~\cref{tab:device_aware_fids}. \framework{}-generated circuits are run without any optimization, but the device-unaware circuits are optimized using level 3 of the Qiskit compiler and with SABRE~\cite{li2018sabre}, a state-of-the-art qubit mapping and routing algorithm. There are significant differences between the fidelities of device-aware and device-unaware circuits, demonstrating that using \framework{}'s device-aware circuit generation not only eliminates the need for qubit mapping, but also results in circuits with higher noise robustness.}}

\begin{table}[h]
  \centering
\setlength{\tabcolsep}{0.35cm} 
\renewcommand{\arraystretch}{1.2}
\begin{center}
    \caption{\imp{\new{Comparison of Elivagar-generated (no optimization) and SABRE~\cite{li2018sabre}-optimized device-unaware random circuits (Qiskit compiler level 3).}}}
    \label{tab:device_aware_fids}
    \begin{tabular}{l c c c}
        \toprule
         Policy & 2Q gates & \makecell{2Q gates after\\compilation $\downarrow$} & Fidelity $\uparrow$\\
        %\hline
        \midrule
        \multicolumn{4}{c}{\textbf{IBM-Geneva (27 qubits)}}\\
         \midrule
        \imp{SABRE} & \imp{6.48} & \imp{15.24} & \imp{0.615}\\
        \imp{\framework{}} & \imp{6.48} & \imp{6.48} & \imp{0.714}\\
        \midrule       
        \multicolumn{4}{c}{\textbf{IBMQ-Kolkata (27 qubits)}}\\
        \midrule
        \imp{SABRE} & \imp{9.52} & \imp{22.16} & \imp{0.741}\\
        \imp{\framework{}} & \imp{9.52} & \imp{9.52} & \imp{0.848}\\
        \midrule
        \multicolumn{4}{c}{\textbf{IBMQ-Mumbai (27 qubits)}}\\
        \midrule
        \imp{SABRE} & \imp{9.75} & \imp{25.00} & \imp{0.634}\\
        \imp{\framework{}} & \imp{9.75} & \imp{9.75} & \imp{0.804}\\
        \bottomrule
    \end{tabular}
    \end{center}
    % \vspace*{-0.8cm}
\end{table}

\subsection{Searching for data embeddings}
% \vspace{-0.1cm}
\label{sec:embeddings_comparision}

\imp{In order to demonstrate the benefits of co-searching for a data embedding along with the \new{parametric} portion of a circuit, we compare \framework{} using generated data embeddings with versions of \framework{} that use fixed IQP embeddings~\cite{havlek2019suplearninginquantumenhancedfeaturespaces} and fixed angle embeddings~\cite{qml} for all candidate circuits. We compare the \new{three versions of \framework{} on 5 QML tasks}, and \new{eliminate the effect of noise by ranking circuits solely according to $\textrm{Rep}(C)$ and reporting performance on a noiseless simulator}.~\cref{fig:fixed_vs_searched_embedding} shows the results obtained. \new{The version \framework{} using generated embeddings} performs 2.01x better than \framework{} with fixed IQP embeddings, and 1.26x better than \framework{} using fixed angle embeddings \new{on average}. \new{These results validate the effectiveness of our candidate generation strategy and show that searching over data embeddings is the primary reason for \framework{} ourperforming QuantumNAS.}}
% While we do not expect this advantage to be significant for every QML task, since QML tasks can be constructed to ensure that using a certain embedding results in optimal performance~\cite{nature_communication_2021_power_of_data_qml}, these results illustrate the potential of data-dependent embeddings as a means of unlocking performance gains over a broad range of real-world QML tasks.

\begin{figure}[t]
    % \vspace{-0.1in}
    \centering
    \includegraphics[width=\columnwidth]{figs/perf_analysis/fixed_vs_Seafched_embedding.png}
    \caption{\new{Performance of \framework{} using searched versus fixed data embeddings.} Absolute values of \new{test MSE loss} of \framework{} using a fixed IQP embedding are given below task labels.}
    \label{fig:fixed_vs_searched_embedding}
    % \vspace{-0.2in}
\end{figure}

%let me see
%yes, Yes
% okay awesome
\subsection{Constructing composite scores to rank circuits}

%We discuss the importance of both parts of our predictor of circuit performance $\textrm{Score}(C)$, \metrictwo{} and \metricone{}.
%We observe that while \metricone{} is a strong predictor of circuit performance on ideal devices, its predictive power weakens when used to predict the performance of circuits on noisy devices, as it does not incorporate any noise information. \MT{}, in contrast, is strongly correlated with circuit noise robustness, but is completely uncorrelated with circuit performance. 
%Using either of these predictors alone to predict the performance of circuits on noisy devices is insufficient, as information about both the learning ability and noise robustness of a circuit is required to accurately characterize its performance. 
% Since we compute \MT{} for all circuits in to perform noise-guided circuit rejection (see~\cref{sec:clifford_noise}), this step does not require any additional computation. 
\Metricone{} and \MT{} are strong predictors for performance and noise robustness, respectively.
By combining them to construct a composite score $\textrm{Score}(C)$, we can create a predictor that is aware of both \new{circuit performance} and noise robustness. The correlations corresponding to \MT{}, \metricone{}, and the composite score $\textrm{Score}(C)$ for three different task-device combinations are shown in~\cref{tab:metrics_correlations}. On average, the correlation between $\textrm{Score}(C)$ and \new{circuit performance} is about 15\% stronger than that of $\textrm{Rep}(C)$, demonstrating that combining information on circuit noise robustness and learning ability enables more accurate predictions of circuit performance on noisy devices than using either predictor alone.

\subsection{Sources of runtime speedup}
\label{sec:source_of_speedup}
The speedup of \framework{} over QuantumNAS comes from (1) using \metricone{} for performance evaluation, (2) early rejection of low-fidelity circuits, and (3) eliminating the circuit-mapping co-search by directly generating device-aware circuits. \new{Using \metricone{} speeds up \framework{} by 16$\times-$44$\times$ for the QML tasks in~\cref{sec:evaluation}, growing with problem size. Since we use conservative CNR hyperparameter values(see~\cref{sec:elivagar-hyperparams}), the speedup due to early rejection for all tasks is 2$\times$. Eliminating the circuit-mapping co-search provides a speedup of 1.4$\times-$11.7$\times$, increasing with problem size.}

==> v1/results.tex <==
\section{Results}
\label{sec:evaluation}
% In this section, we compare \framework{} with competing methods in terms of the performance of resulting circuits and resource efficiency. 

\subsection{Performance}
\cref{fig:main_results} shows results obtained on 8 different QML tasks, using noise models of \new{OQC Lucy,  Rigetti Aspen-M-2, IBM-Nairobi, and IBMQ-Manila. All plots in~\cref{fig:main_results} show the accuracy of competing methods and \framework{} relative to the human designed baseline.}

\framework{} achieves the best performance out of all competing methods considered in all tasks except for Vowel-4. On average, \framework{} achieves \perfgain{} higher accuracy than the best competing method (QuantumNAS) and \perfgainhuman{} higher accuracy than the human-designed baseline.

%The surprisingly strong performance of randomly generated circuits compared to QCS methods such as QuantumNAS (RZX + XX) can be attributed to the fact that we generate random circuits using variational gates from a much larger gate set ($\{ RY, RX, RZ, CX, CZ, CRY, CRX, CRZ\}$) than is used by QuantumNAS (RZX + XX), which can significantly impact circuit performance, as demonstrated in~\cite{wang2021quantumnas}, which showed wide variations between the results obtained by QuantumNAS when using different gate sets.

\subsection{Runtime speedup}
\framework{} requires only a fraction of the quantum resources (measured by number of circuit executions) used by QuantumSupernet and QuantumNAS. \new{The reduction of circuit executions of \framework{} also results in near-equivalent runtime speedups since the runtimes of QCS frameworks are dominated by quantum circuit executions.} As shown in~\cref{tab:resources}, \framework{} enjoys an average speedup of 186$\times$ (up to 1048$\times$) over QuantumNAS and 349$\times$ (up to 2001$\times$) over QuantumSupernet, respectively. Importantly, \framework{} shows more substantial runtime advantages for larger QML tasks, indicating its more favorable scaling.
\begin{table}[h]
  \centering
\setlength{\tabcolsep}{0.33cm} 
\renewcommand{\arraystretch}{1.2}
\begin{center}
\caption{Runtime speedup relative to QuantumSupernet (\textit{higher is better})}
    \label{tab:resources}
    \begin{tabular}{l c c}
    \toprule
    Benchmark & QuantumNAS & \textbf{\framework{}}\\
    \midrule
    Moons (16 param) & 1.79x & \textbf{80x} \\
    Vowel-4 (40 param.) & 1.93x & \textbf{150x} \\
    Vowel-2 (32 param.) & 1.91x & \textbf{200x} \\
    Bank (20 param.)& 1.92x & \textbf{213x} \\
    MNIST-2 (20 param.) & 1.83x & \textbf{333x} \\
    FMNIST-2 (32 param.) & 1.89x & \textbf{533x} \\
    FMNIST-4 (24 param.) & 1.86x & \textbf{1201x} \\
    MNIST-4 (40 param.) & 1.91x & \textbf{2001x} \\
    \midrule
    \textbf{GMean} & \textbf{1.88x} & \textbf{349x}\\
    \bottomrule
    \end{tabular}
    \end{center}
    % \vspace*{-0.8cm}
\end{table}

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.48\textwidth]{figs/results/speedups.png}
%     \caption{The speedups (quantum resource efficiency improvements)  of \framework{} and QuantumNAS relative to QuantumSupernet for each QML task. The dataset sizes of the QML tasks are in the ascending order.}
%     \label{fig:speedups}
%     \vspace*{-0.3cm}
% \end{figure}


==> v1/search_algorithm.tex <==


\begin{figure*}[t]
    \centering
     \begin{subfigure}{0.14\textwidth}
        \includegraphics[width=1\columnwidth]{figs/search_algo/orignla circ@3x.png}
       \caption{}
        \label{fig:original_circuit_sec_5}
    \end{subfigure}
        \hfill
     \begin{subfigure}{0.14\textwidth}
\includegraphics[width=1\columnwidth]{figs/search_algo/clifford circ1@3x.png}
       \caption{}
        \label{fig:clifford_circuit_sec_5}
    \end{subfigure}
        \hfill
         \begin{subfigure}{0.31\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figs/search_algo/real_device_runsn.png}
        \caption{}
        \label{fig:clifford_correlation_realdevice}   
    \end{subfigure}
     \hfill
         \begin{subfigure}{0.31\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figs/search_algo/aspen_sim.png}
        \caption{}
        \label{fig:clifford_correlation_simulator}   
    \end{subfigure}
    \caption{(a) A circuit and (b) a Clifford replica of the circuit. \new{\MT{} is strongly correlated with circuit fidelity, as demonstrated using circuits run on (c) IBMQ-Kolkata and IBMQ-Guadeloupe, and a (d) noise model of Rigetti Aspen-M-2.}}
    \label{fig:correlations}
    % \vspace*{-0.4cm}
\end{figure*}

\section{Noise-guided candidate rejection}
\label{sec:clifford_noise}

One of the key insights of \framework{} is that evaluating circuit robustness is much simpler than predicting the performance of a circuit on a QML task. Leveraging this insight, \framework{} reduces the total number of performance evaluations required via the identification and early rejection of low-fidelity circuits. To achieve this, \framework{} defines a \new{predictor}, \textit{\metrictwo{}} (\MT{}), that cheaply and accurately estimates the fidelity of candidate variational circuits. 

Clifford circuits are a class of quantum circuits that can be efficiently simulated on classical computers~\cite{PhysRevLett_cliffordSimulation}. Thus, the fidelity of noisy Clifford circuit executions on real quantum hardware can be calculated efficiently by comparing their noisy outputs with noiseless classical simulation results. This idea enables efficient fidelity estimation for a circuit by using the fidelity of its \emph{Clifford replicas} as a proxy~\cite{Knill_2008_randomizedBenchmarking}. While prior works use Clifford replicas to create enhanced circuit compilation passes~\cite{das2021adapt, das2022imitationgame, QAFCA} and characterize device noise~\cite{ravi2022cliffordcanarycircuits}, \framework{} uses Clifford circuits to identify noise-robust circuits for QML. First, we explain how Clifford replicas are constructed, how \MT{} is defined and computed, and elaborate on the resources required to compute \MT{}. Then, we demonstrate the effectiveness of \MT{} by showing the correlation between the \MT{} and circuit fidelity.

\vspace{2pt}
\subsection{Creating Clifford replicas} To create a Clifford replica of a circuit, we replace each of its single-qubit gates with a randomly chosen single-qubit Clifford gate (H, S, Z, X, Y) and its 2-qubit gates with the CNOT gate, which is also a Clifford gate. Figure \ref{fig:original_circuit_sec_5} and \ref{fig:clifford_circuit_sec_5} show a circuit and one of its Clifford replicas. \new{\imp{Since Clifford replicas use the same structure as the original circuit, circuit properties such as the proportion of 2-qubit gates and depth are preserved.} To reliably estimate noise robustness, \framework{} creates multiple Clifford replicas and uses the fidelities of all the constructed replicas to estimate circuit noise robustness.} We empirically find that as analyzing as few as 16 Clifford replicas can provide an accurate characterization of circuit noise robustness.
\vspace{2pt}

\subsection{Computing CNR} To compute the \MT{} for a circuit, \framework{} first collects the noisy outputs $P_{\textrm{noisy}}$ obtained by executing the \new{generated Clifford replicas on the target quantum device. Then, it executes the same Clifford replicas on a classical simulator to obtain the ideal noiseless outputs $P_{\textrm{noiseless}}$.} To evaluate the fidelity of the Clifford replicas, \framework{} calculates the Total Variation Distance (TVD) between the noisy and noiseless outputs, given by
\vspace{2pt}

\begin{equation}
\label{eq:tvd}
\new{\textrm{TVD} = \frac{1}{2} \sum_{i \in [2^{n_q}]} | P_{\textrm{noiseless}}(|i\rangle) - P_{\textrm{noisy}}(|i\rangle) |.}
\end{equation}
The fidelity of the replica is computed as $\textrm{Fid} = 1- \textrm{TVD}$. $\textrm{CNR}(C)$, the \metrictwo{} for circuit $C$, is defined as the average fidelity of the \new{$M$ Clifford replicas} $C_{Ri}$:
\vspace{2pt}
\begin{equation}
    \textrm{CNR}(C) = \frac{1}{M}\sum ^{M}_{i=1} \textrm{Fid}(P^{C_{Ri}}_{\textrm{noiseless}},\: P^{C_{Ri}}_{\textrm{noisy}}). 
    \label{eq:cnr}
\end{equation}

\subsection{Candidate circuit rejection}
After computing the \MT{} of candidate circuits, \framework{} ranks circuits by CNR, and by default rejects the circuits with \MT{} values that are less than a threshold of 0.7, or outside the top 50\% of all candidates. However, the threshold and the percentage of candidates to reject can be set by users of \framework{} as hyperparameters. All rejected circuits require no performance evaluation, leading to reduced resource requirements. Depending on the device noise-level and threshold values, this rejection step can reduce the circuit executions required by \framework{} significantly. For example, when searching for a 250-parameter circuit on IBMQ-Manila using a \MT{} threshold of 0.9, \framework{} can reject 95\% of candidate circuits, achieving an almost 20x reduction in the total number of circuit executions. 

\begin{figure*}[t]
    \centering
     \begin{subfigure}{0.5\textwidth}
        \includegraphics[width=\columnwidth]
        {figs/candidate_eval/mappign diag@3x.png}
       \caption{}
        \label{fig:rep_cap_diag}
    \end{subfigure}
        \hfill
    \begin{subfigure}{0.48\textwidth}
        \centering
        \includegraphics[width=0.49\columnwidth]{figs/candidate_eval/spuernet.png}
        \includegraphics[width=0.49\textwidth]{figs/candidate_eval/fmnist_2.png}
        \caption{}
        \label{fig:rep_cor1}   
    \end{subfigure}
     \hfill

    \caption{(a) \Metricone{} measures the degree of intra-class similarity and inter-class separation of the quantum states created by a circuit. Circuit 1 has a higher \metricone{}, and so is likely to perform better than Circuit 2. (b) Predictor correlations with circuit performance on the FMNIST-2 dataset. $\textrm{Rep}(C)$ is as strong a predictor of circuit performance as a SuperCircuit, despite not involving gradient computation.}
    \label{fig:correlations}
    % \vspace*{-0.4cm}
\end{figure*}

In comparison, \new{SuperCircuit-based QCS works} conflate \new{the evaluation of circuit noise robustness and circuit performance}, \new{making the identification of low-fidelity circuits unnecessarily expensive.} In these methods, the performance of all candidate circuits is evaluated using a validation data set $\mathcal{X_{\text{valid}}}$ on a noisy device. This requires executing $|\mathcal{X_{\text{valid}}}|$ circuits for every candidate circuit. For larger problems, $|\mathcal{X_{\text{valid}}}|$ can be significantly greater than the constant number of circuits required to compute \MT{}, making the identification of low performing circuits unnecessarily expensive.
%In~\cref{sec:perf_analysis}, we detail the improvement by \framework{} due to early rejection.

%compared to computing \metricone{} (outlined in~\cref{sec:metrics_explanations}), which requires 512 circuit executions per class in the input dataset. Computing \metrictwo{} is 16 times cheaper than computing \metricone{} on a 4-class dataset, and 40 times cheaper than computing \metricone{} on a 10-class dataset, making it ideal as a means of cheaply rejecting candidate circuits early in the search process.

Figure~\ref{fig:clifford_correlation_realdevice} and~\ref{fig:clifford_correlation_simulator} show the correlation between the \MT{} and the fidelity of circuits executed on IBMQ-Guadalupe and IBMQ-Kolkata, and a \new{noise model of Rigetti Aspen-M-2, respectively, for candidate circuits generated via~\cref{alg:candidategen}. The fidelity of circuits is computed by averaging the fidelities of multiple copies of a circuit executed with different inputs data and variational parameter values.} In all cases, the \MT{} computed using Clifford replicas is highly predictive of the true noise robustness of the circuit.
\vspace{0.2cm}
\begin{hintbox}{\color{white}\textbf{Insight 3: Early rejection of low-fidelity circuits}}
Noise robustness evaluation is simpler than performance evaluation. Evaluating noise robustness first using \metrictwo{} enables early rejection of low-fidelity circuits, reducing evaluation costs.
\end{hintbox}

\ignore{
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.5\textwidth]{figs/candidate_eval/mappign diag@3x.png}
        
    \caption{\YS{draw a measurement operation on the 1st qubit; the Sim in the fig should be Rep(C)?} \Metricone{} measures the degree of intra-class clustering and inter-class separation of the final quantum states for a variational circuit. Compared to Circuit 2, the output quantum states of the same color labels in Circuit 1 are more clustered and that of opposite color labels are more distant. Thus, Circuit 1 has a higher \metricone{}, and is likely to have a better performance.}
  
    %Both Circuit 1 and Circuit 2 are 4-qubit circuits trained on the 2-class dataset shown on the left, with the expectation values obtained by measuring the first qubit taken as the output of the circuits. The representations of the input data using Circuit 1 (shown as points on the Bloch sphere) are much better than those constructed using Circuit 2, since the representations of samples from the same class are very similar, and the representations of points from different classes are dissimilar, as shown by the similarity scores next to each set of representations. On the other hand, the representations learned by Circuit 2 do not reflect the label structure of the dataset, and so Circuit 2 learns a bad classification boundary for the dataset.}
    % \vspace*{-0.4cm}
    \label{fig:rep_cap_diag}
\end{figure}
 } 
 
\ignore{The motivation behind using Clifford replicas instead of running the circuit itself with randomly chosen inputs and parameters is twofold:
\begin{itemize}
    \item Noiseless simulation of quantum circuits on classical hardware is exponentially hard in general, but circuits comprised solely of Clifford gates can be simulated efficiently, which reduces the cost of estimating \metrictwo{} for a circuit drastically.

    \item The structure of a circuit is more important for determining fidelity than the exact gates themselves, resulting in the average noise robustness of multiple Clifford replicas being almost perfectly representative of the noise robustness of the original circuit.
\end{itemize}}

==> v1/search_space.tex <==
\section{Candidate circuit generation}
\label{sec:circuit_generation}

% In this section, we elaborate on our candidate generation process, which can be broken down into two separate steps: generating noise- and device-aware circuits, and constructing variable data embeddings for cnaidate circuits.

%As discussed in~\cref{sec:intro}, SuperCircuit-based candidate circuit generation leads to several issues: (1) human-designed SuperCircuits narrow the search space by restricting candidate circuit structures and data-embedding gates; (2) sampling candidate circuits from a topology-agnostic SuperCircuit necessitates an expensive circuit-qubit mapping co-search and cannot guarantee the elimination of quantum SWAP gates to achieve hardware-efficiency.

To overcome the issues of SuperCircuit-based circuit generation discussed in~\cref{sec:intro}, \framework{} directly generates candidate circuits and data embeddings based on target device topology via a noise-guided sampling policy shown in~\cref{alg:candidategen}. This approach has the following advantages over SuperCircuit-based methods: \new{1) generating circuits based on device topology ensures that no SWAP gates are inserted, ensuring hardware-efficiency and improving circuit fidelity; 2) circuits are generated along with optimal qubit mappings, eliminating the need for an expensive circuit-mapping co-search; 3) noise-guided sampling further boosts the average fidelity of candidate circuits;} 4) generating varied data embeddings for candidate circuits can significantly improve the performance of the selected circuit. \imp{As a result, circuits generated by \new{\framework{} have \new{18.7\%} higher fidelity than device-unaware circuits optimized using SABRE~\cite{li2018sabre} (\cref{sec:device_aware_gen}). Furthermore, \framework{} performs up to 2.01$\times$ better on QML tasks when searching for an optimal data embedding than when using a fixed data embedding (\cref{sec:embeddings_comparision}).}}

\subsection{Noise-Guided Candidate Circuit Generation}
As shown in~\cref{alg:candidategen}, \framework{} first chooses a subgraph from the set of connected subgraphs of the device topology. Then, \framework{} samples a list of 1- and 2-qubit gates to form the circuit. Gate placement choices are guided by device connectivity, noise information such as qubit coherence times, 1- and 2-qubit gate fidelities, readout fidelities, and the current circuit structure. Following the convention of prior works in classical neural architecture search~\cite{liu2018darts, yang2019gdas}, \framework{} uses the Softmax distribution to sample the subgraph, gate placements, and the qubits to measure instead of simply choosing the top ranked option based on noise and device information. The usage of a Softmax distributions is done solely to promote circuit diversity, and any other suitable distribution could be used as well. Here we show the definition of the distribution $\textrm{P}_{\text{meas}}$ on line 13 of~\cref{alg:candidategen} that chooses a qubit to measure among the $|V^{(S)}|$ qubits in the chosen subgraph $S$:
\begin{equation}
    \new{\textrm{P}_{\text{meas}}(q \: | \: R_{E^{(S)}}) = \frac{\text{exp}(\frac{R_q}{\tau})}{\sum_{q' \in V^{(S)}} \text{exp}(\frac{R_{q'}}{\tau})}.}
\end{equation}
\new{Here $R_q$ is the readout fidelity of the qubit $q \in V^{(S)}$, and} $\tau$ is a parameter that controls the uniformity of $\textrm{P}$ and thus the diversity in the candidate circuits generated.

\begin{algorithm}[t]
%\setstretch{1}
\SetAlgoLined
 
    \KwIn{Device topology graph ${G}(\{V_i\}, \{E_j\})$; Qubit readout errors $\{R_i\}$; Qubit coherence times $\{\mathrm{T1}_i \}, \{\mathrm{T2}_i\}$; 2-qubit gate fidelity $\{Q_j\}$; Output circuit configuration $O_{\text{conf}}$.}
    \KwOut{Candidate circuit $C$.}

    Sample a set of connected subgraphs $\{S_i\}$ with \new{$V^{(S_i)} = O_{\text{conf}}.n_q \: \forall_i$} from $G$;
    
    \new{Select a subgraph $S(V^{(S)}, E^{(S)})$ from distribution 
    $\textrm{P}_{\{S_i\}}(S \: | \: R_{V^{(S)}}, \mathrm{T1}_{V^{(S)}}, \mathrm{T2}_{V^{(S)}}, Q_{E^{(S)}})$\;}

    Initialize $C$ as an empty circuit\;

    Randomly sample a list $L_{\text{op}}$ of 1-qubit and 2-qubit gates based 
    on \new{$O_{\text{conf}}.n_{\text{params}}$ and $O_{\text{conf}}.n_{\text{embeds}}$\;}
 
    \For{$op$ in $L_{\text{op}}$}{
        \If{$op$ is a 1-qubit gate}{
            Select a qubit $q \in V^{(S)}$ from distribution \new{$\textrm{P}_{1\text{q}}(q \: | \: C, \mathrm{T1}_{q}, \mathrm{T2}_{q})$\;}
           
            Append $op(q)$ to $C$\;
         }
         
        \If{$op$ is a 2-qubit gate}{
            Select an edge $e = (q_0, q_1) \in E^{(S)}$ from distribution \new{$\textrm{P}_{2\text{q}}(e \: | \: C, \mathrm{T1}_{q_0}, \mathrm{T1}_{q_1}, \mathrm{T2}_{q_0}, \mathrm{T2}_{q_1}, Q_e)$\;}
              
            Append $op(q_0, q_1)$ to $C$\;
        }
    }

    Select a set $q_{\text{meas}}$ of $O_{\text{conf}}.n_{\text{meas}}$ qubits in $V^{(S)}$ from distribution \new{$\textrm{P}_{\text{meas}}(q \: | \: R_{E^{(S)}})$\;}
    
    Append MEASURE($q_{\text{meas}}$) to $C$\;
    
    Randomly designate $O_{\text{conf}}.n_{\text{embeds}}$ parametric gates in $C$ for use as data embedding gates\;
    
    \Return $C$;
    \caption{Generate device-aware circuits}
    \label{alg:candidategen}
    % \vspace{-0.4cm}
    \vspace{-4pt}
\end{algorithm}

\begin{hintbox}{\color{white}\textbf{Insight 1: Generating device-aware circuits}}
Generating candidate circuits based on device topology and noise data eliminates the need for an expensive circuit-mapping co-search, improves circuit noise robustness, and ensures hardware-efficiency.  
\end{hintbox}

\vspace{-0.2cm}
\subsection{Generating Data Embeddings}
\label{sec:data_embeddings_strategy}
%As discussed in~\cref{sec:data_embedding}, d
% Data embeddings are a key determinant of circuit performance~\cite{schuld2021encodingexpressivity, schuld2022fourierinterpolation, sweke2021encodingdependentbounds} and thus constitute an important part of \framework{}'s search space. However, searching for data embeddings can incur significant costs due to the exponential number of possible data embeddings. To maintain resource efficiency, \framework{} employs a low-cost strategy to generate data embeddings: as part of the circuit generation process, \framework{} designates a portion of the gates in candidate circuits as data embedding gates (line 14 in~\cref{alg:candidategen}). The number of data embedding gates depends on the dimensionality of the QML dataset the circuit will be used with. These gates are randomly assigned one dimension of the data to embed, as opposed to being used as parametric gates for training.
% During the circuit performance evaluation step (\cref{sec:metrics_explanations}) of \framework{}, the effectiveness of these data embeddings are evaluated together with the trainable variational parts of candidate circuits. The feedback from the performance evaluation process enables optimization of the data embedding in a task-specific manner. \new{Despite its simplicity, \framework{} using data embeddings generated via this strategy performs significantly better on QML tasks: 2.01$\times$ better than \framework{} using a fixed IQP embedding, and 1.26$\times$ better than when using a fixed angle embedding, as shown in~\cref{sec:embeddings_comparision}.}

\framework{} employs a low-cost strategy to generate data embeddings: a portion of the gates in generated circuits are designated as data embedding gates (line 14 in~\cref{alg:candidategen}), and each gate is randomly assigned one dimension of the input data to embed. The number of data embedding gates depends on the QML task the circuit will be used for.
During the circuit performance evaluation step (\cref{sec:metrics_explanations}) of \framework{}, the effectiveness of these data embeddings are evaluated together with the trainable variational parts of candidate circuits. The feedback from the performance evaluation process enables optimization of the data embedding in a task-specific manner. Despite its simplicity, \framework{} using data embeddings generated via this strategy performs significantly better on QML tasks: 2.01$\times$ better than \framework{} using a fixed IQP embedding, and 1.26$\times$ better than when using a fixed angle embedding, as shown in~\cref{sec:embeddings_comparision}.

\begin{hintbox}{\color{white}\textbf{Insight 2: Searching for optimal data embeddings}}
\new{Using optimized data embeddings significantly boosts performance over QCS methods with fixed embeddings.}
\end{hintbox}


==> v2/9_performance_analysis.tex <==
\section{Performance Analysis}
\label{sec:perf_analysis}

% just headings to remind me what to add
\subsection{Benefits of device-aware circuit generation}
\label{sec:device_aware_gen}

To analyze \framework{}'s circuit generation strategy, we compare device-aware circuits generated via \cref{alg:candidategen} with randomly generated, device-unaware circuits. We generate pairs of device-aware and -unaware circuits with the same number of 1- and 2-qubit gates before compilation to ensure a fair comparison. Average circuit characteristics are shown in~\cref{tab:device_aware_fids}. Device-aware circuits are run unoptimized, but the device-unaware circuits are optimized using level 3 of the Qiskit compiler and SABRE~\cite{li2018sabre}. Device-aware circuits have significantly higher fidelities on all devices (18.9\% higher on average), indicating that \framework{}'s circuit generation strategy not only eliminates the need for a circuit-mapping co-search, but also boosts circuit fidelity.

\begin{table}[t]
  \centering
\setlength{\tabcolsep}{0.33cm} 
\renewcommand{\arraystretch}{1.1}
\begin{center}
\caption{Speedup relative to QuantumSupernet (\textit{higher is better})}
    \label{tab:resources}
    \begin{tabular}{l c c}
    \toprule
    Benchmark & QuantumNAS & \textbf{\framework{}}\\
    \midrule
    Moons (16 param.) & 1.79x & \textbf{80x} \\
    Vowel-4 (40 param.) & 1.93x & \textbf{150x} \\
    Vowel-2 (32 param.) & 1.91x & \textbf{200x} \\
    Bank (20 param.)& 1.92x & \textbf{213x} \\
    MNIST-2 (20 param.) & 1.83x & \textbf{333x} \\
    FMNIST-2 (32 param.) & 1.89x & \textbf{533x} \\
    FMNIST-4 (24 param.) & 1.86x & \textbf{1201x} \\
    MNIST-4 (40 param.) & 1.91x & \textbf{2001x} \\
    \midrule
    GMean & 1.88x & \textbf{349x}\\
    \bottomrule
    \end{tabular}
    \end{center}
    \vspace*{-0.5cm}
\end{table}

\begin{table}[h]
  \centering
\setlength{\tabcolsep}{0.22cm} 
\renewcommand{\arraystretch}{1.1}
\begin{center}
\caption{Spearman R correlations with circuit performance for different benchmark-device combinations (\textit{lower is better})}.
    \label{tab:metrics_correlations}
    \begin{tabular}{ l c c c}
    \toprule
    Dataset & FMNIST-2 & Vowel-2 & FMNIST-4\\
    Device & IBMQ-Lima & IBMQ-Quito & IBM-Nairobi\\
    \midrule
    \MO{}$(C)$ & -0.675 & -0.572 & -0.516\\
    % $R(\textrm{CNR}(C), \mathcal{L}_{C})$ & -0.149 & -0.094 & -0.359\\
    $\textbf{Score}\textbf{(\textit{C})}$ & \textbf{-0.703} & \textbf{-0.678} & \textbf{-0.663}\\
    \bottomrule
    \end{tabular}
    \end{center}
    \vspace*{-0.3cm}
\end{table}

\begin{table}[t]
  \centering
\setlength{\tabcolsep}{0.34cm} 
\renewcommand{\arraystretch}{1.1}
\begin{center}
    \caption{Comparing Elivagar-generated (no optimization) and device-unaware random circuits (SABRE~\cite{li2018sabre} + Qiskit compiler level 3).}
    \label{tab:device_aware_fids}
    \begin{tabular}{l c c c}
        \toprule
         Policy & 2Q gates & \makecell{2Q gates after\\compilation $\downarrow$} & Fidelity $\uparrow$\\
        \midrule
        \multicolumn{4}{c}{OQC Lucy}\\
        \midrule
        \imp{SABRE} & \imp{7.04} & \imp{16.22} & \imp{0.595}\\
        \imp{\textbf{\framework{}}} & \imp{\textbf{7.04}} & \imp{\textbf{7.04}} & \imp{\textbf{0.706}}\\
        \midrule
        \multicolumn{4}{c}{IBM-Geneva}\\
         \midrule
        \imp{SABRE} & \imp{6.48} & \imp{15.24} & \imp{0.615}\\
        \imp{\textbf{\framework{}}} & \imp{\textbf{6.48}} & \imp{\textbf{6.48}} & \imp{\textbf{0.714}}\\
        \midrule       
        \multicolumn{4}{c}{IBMQ-Kolkata}\\
        \midrule
        \imp{SABRE} & \imp{9.52} & \imp{22.16} & \imp{0.741}\\
        \imp{\textbf{\framework{}}} & \imp{\textbf{9.52}} & \imp{\textbf{9.52}} & \imp{\textbf{0.848}}\\
        \midrule
        \multicolumn{4}{c}{IBMQ-Mumbai}\\
        \midrule
        \imp{SABRE} & \imp{9.75} & \imp{25.00} & \imp{0.634}\\
        \imp{\textbf{\framework{}}} & \imp{\textbf{9.75}} & \imp{\textbf{9.75}} & \imp{\textbf{0.804}}\\
        \bottomrule
    \end{tabular}
    \end{center}
    \vspace*{-0.2cm}
\end{table}

\subsection{Benefits of searching for data embeddings}
% \vspace{-0.1cm}
\label{sec:embeddings_comparision}

To demonstrate the benefits of co-searching for data embeddings and variational gates, we compare \framework{} with versions of \framework{} that use fixed angle~\cite{qml} and IQP embeddings~\cite{havlek2019suplearninginquantumenhancedfeaturespaces}. We evaluate the three versions of \framework{} using a noiseless simulator to eliminate the effects of noise.~\cref{fig:fixed_vs_searched_embedding} shows the results obtained. \framework{} using generated data embeddings performs 2.01x better than \framework{} with fixed IQP embeddings, and 1.26x better than \framework{} using fixed angle embeddings on average. This validates our data embedding generation strategy, and shows that searching over data embeddings is the primary reason for \framework{} outperforming QuantumNAS.

\begin{figure}[h]
    % \vspace{-0.1in}
    \centering
    \includegraphics[width=\columnwidth]{figs/perf_analysis/fixed_vs_Seafched_embedding_2.png}
    \caption{Performance of \framework{} using generated versus fixed data embeddings. Absolute values of test MSE of \framework{} using a fixed IQP embedding are given below task labels.}
    \label{fig:fixed_vs_searched_embedding}
    % \vspace{-0.2in}
\end{figure}

\subsection{Breakdown of performance gains}

\subsection{Compatibility with other QML frameworks}
\framework{} can be coupled with 

\subsection{Sources of runtime speedup}
\label{sec:source_of_speedup}
The speedup of \framework{} over QuantumNAS comes from (1) using \metricone{} for performance evaluation, (2) early rejection of low-fidelity circuits, and (3) eliminating the circuit-mapping co-search by generating device-aware circuits. Using \metricone{} speeds up \framework{} by 16$\times-$44$\times$ for the benchmarks in~\cref{sec:evaluation}, growing with problem size. Since we use conservative CNR hyperparameter values, the speedup due to early rejection for all tasks is 2$\times$. Eliminating the circuit-mapping co-search provides a speedup of 1.4$\times-$11.7$\times$, growing with problem size.

\subsection{Constructing composite scores for circuits}
$\text{Score}(C)$, which we use to rank circuits, combines both \MT{} and \MO{} (\cref{sec:combining_metrics}). To determine whether $\text{Score}(C)$ ranks circuits better than \MO{} alone, we compare how strongly $\text{Score}(C)$ and \MO{} are correlated with trained circuit performance on noisy hardware. As can be seen in \cref{tab:metrics_correlations}, $\text{Score}(C)$ is a stronger predictor of circuit performance than \MO{} alone, validating our choice of using both circuit learning ability and noise robustness to rank circuits.

==> v2/background_v2.tex <==
%\newpage %%% do not move this--- I need to estimate the space
\section{Background}
\label{sec:background}
\subsection{Execution of Quantum Programs on NISQ Computers}
% To run a quantum program, compilers (1)~\textit{map} the program qubits on to the physical qubits of the target quantum device and (2)~\textit{translates} the high-level program instructions on to low-level device-compliant native gates. Unfortunately, noisy quantum devices and imperfections in quantum operations make program executions susceptible to computational errors. 

In the NISQ era, noisy quantum devices and imperfect quantum operations make program executions susceptible to computational errors. Moreover, most NISQ devices have limited connectivity between qubits. To overcome this, a circuit  \textit{routing} step is required to execute operations between non-adjacent qubits. This is performed using quantum SWAP gates, as shown in~\cref{fig:swap}. SWAP operations are usually implemented using 3 imperfect physical 2-qubit gates, and thus are expensive and error-prone. Prior works~\cite{murali2020crosstalk, das2021adapt, ravi2022cliffordcanarycircuits, tannu2022hammer} show that circuit fidelity can be improved by leveraging circuits that require less SWAP operations or with structures that are more robust to various device error sources.

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.99\textwidth]{figs/framework/overview@3x.png}
        
    \caption{An overview of \framework{}.}
    % \vspace*{-0.2cm}
    \label{fig:framework_overview}
\end{figure*}
 
\subsection{Quantum Machine Learning}
\label{sec:qml_intro}
%, shown in \cref{fig:qml}
% (1)~\textit{data embedding} in which the input training data is encoded into the quantum states manipulated by a variational circuit, 
\subsubsection{Variational circuits}
QML uses variational circuits to perform machine learning tasks. Variational circuits for QML consist of three parts: a trainable variational subcircuit, a set of data embedding gates, and a set of measurement operations. Trainable variational subcircuits often include parametric 1- and 2-qubit gates (ex. RY$(\theta)$, where $\theta$ is a trainable parameter) and some non-parametric gates (ex. CX). Data embedding gates are used to encode classical data into quantum states that can be manipulated by variational circuits. Measurement operations are performed on a subset of the qubits operated on by a circuit to obtain circuit outputs for further processing. 

\subsubsection{Data embedding gates}
\label{sec:data_embedding}

While current QCS methods focus on optimizing the variational portion of a QML circuit, the data embedding used is a key determinant circuit performance \cite{schuld2022fourierinterpolation, schuld2021encodingexpressivity, schuld2021qmlmodelsarekernelmethods, sweke2021encodingdependentbounds}. We use a simple 1-qubit example to illustrate this. As seen in ~\cref{fig:embedding}, two 1-qubit variational circuits with the same parametric gates (U3$(\vec{\theta_1})$ and U3$(\vec{\theta_2})$) but different embeddings (RX$(x)$ and RY$(x)$, versus RX$(x)$ only) exhibit completely different performance when used to learn a simple sinusoidal function. The theory developed in~\cite{schuld2021encodingexpressivity, schuld2022fourierinterpolation} emphasizes the need to use a well-suited data embedding to accurately learn any target function. Thus, identifying such data embeddings for a given QML task is crucial for high performance.

Unfortunately, finding effective data embeddings is challenging due to the large search space. Existing QCS frameworks rely on fixed embedding schemes, such as angle~\cite{qml} or IQP~\cite{havlek2019suplearninginquantumenhancedfeaturespaces} embeddings, and place these embedding gates at the beginning of every circuit. This can lead to poor performance due to the mismatch between the QML task and the embedding used
.
\subsubsection{Training variational circuits}
As illustrated in~\cref{fig:qml}, the training process of variational circuits involves iterating between circuit executions and a classical optimization algorithm. However, training variational circuits is more expensive than training a classical ML model due to the increased cost of gradient computation on quantum hardware. Classically, gradients can be computed in constant time via Automatic Differentiation (AD)~\cite{ad_survey}. However, AD is not feasible on quantum computers since intermediate quantum states cannot be manipulated or copied~\cite{NielsenChuang, nocloning}. Gradient-based optimization for QML uses parameter-shift rules \cite{schuld2019analyticgradients, wierichs2022parametershift} for computing gradients. Parameter-shift rule based methods evaluate the gradient of a single parameter $\theta$ by running two circuits with shifted parameters $\theta+s$ and $\theta-s$ ($s$ is a constant), and computing the difference. This requires circuit executions linear in the number of circuit parameters, as opposed to the constant scaling of AD methods. Thus, computing gradients in QML scales poorly with circuit size. Current QCS methods use SuperCircuit-based candidate evaluation strategies which rely heavily on gradient computation, and so inherit this unfavourable scaling, leading to large training costs.
